ASKAP J005512.2-255834: A Luminous, Long-Lived Radio Transient at z = 0.1 -- an Orphan Afterglow or an off-nuclear TDE from an IMBH?

We report the discovery of a slowly evolving, extragalactic radio transient, ASKAP J005512.2--255834 (hereafter ASKAP J0055-2558), identified using the Australian SKA Pathfinder in a search for orphan afterglows associated with archival gravitational wave events. Although discovered in this context, there is no evidence that the transient is associated with any known gravitational wave event. Nonetheless, this source exhibits a 20-fold increase in flux density over $<250$ days, and it remains in a declining, detectable state more than 1000 days after the initial detection. Follow-up observations from 0.3 to 9 GHz reveal an evolving spectrum consistent with synchrotron emission. ASKAP J0055-2558 is spatially coincident with a low-mass, star-forming galaxy at redshift $z = 0.116$ ($d_{\rm L}$= 543 Mpc), placing its peak radio luminosity at $\nu L_\nu \sim 10^{39}\,\rm erg\,s^{-1}$. Analysis of its radio light curve, inferred blastwave velocity, energetics, host galaxy properties and the absence of counterparts at other wavelengths suggest that ASKAP J0055-2558 is most consistent with either the late-time phase of an orphan long gamma-ray burst afterglow or a tidal disruption event involving an intermediate-mass black hole spatially offset from the galaxy nucleus. The radio discovery of either of these phenomena is extremely rare, with only a few or no confirmed examples to date.

==> misc.tex <==
The inferred outflow velocity, $\beta$, spans 0.3--0.8$c$, with higher values for conical geometries. This places ASKAP~J0055$-$2558 in the mildly relativistic regime. As the velocity estimates are anchored to the time of first radio detection, they represent upper limits as the launch date would have been earlier. The equipartition energy ranges from $10^{50}$ to $10^{53}$~erg. The observed increase in energy with decreasing velocity is characteristic of engine-driven outflows \citep{2013ApJ...778...18M}, such as  relativistic TDEs \citep[eg., Swift~J1644+57;][]{2018ApJ...854...86E} and GRBs \citep[eg., GRB 030329;][]{2008HEAD...10.0506V}.

In Figure~\ref{Figure:E_gammabeta}, we show the derived blastwave energy as a function of velocity for ASKAP J0055–2558, alongside other transient classes. ASKAP J0055–2558 occupies a phase space more consistent with fast blue optical transients (FBOTs) and the late-time, sub-relativistic evolution of gamma-ray bursts (GRBs) and jetted TDEs, which show mildly relativistic ejecta and energies ranging $10^{50}$–$10^{51}$ erg. The energy and velocity are significantly higher than those of typical core-collapse supernovae, which generally exhibit non-relativistic ejecta and energies around $10^{51}$ erg \citep{2006ApJ...651.1005S,2013ApJ...778...18M}.

The $E_k-\Gamma\beta^k$ profiles for ASKAP J-0055-2558 are significantly shallower than those expected from ordinary supernovae \citep[$k\sim-5.2$;][]{2001ApJ...551..946T} and steeper than the those expected from GRBs \citep[$k\sim-0.4$;][]{2012ApJ...750...68L}. The slopes across ejecta geometries indicate that ASKAP J0055–2558 is broadly consistent with the intermediate regime, characteristic of weak jet-driven explosions, where the jet either fails to fully penetrate the stellar envelope or barely breaks through \citep{2014ApJ...797..107M, 2013ApJ...778...18M} - reflecting a uneven distribution of energy across relativistic and slower ejecta. This supports its classification as a rare, non-thermal, engine-driven explosion—possibly involving a choked or off-axis jet.

% The mildly declining density profile inferred here suggests a structured but non-homogeneous ambient medium, potentially shaped by prior mass-loss episodes or jet–ejecta interactions. Compared to FBOTs, which can exhibit high densities and compact environments , ASKAP~J0055$-$2558 appears to lie on the low-density, extended-envelope end of the spectrum. F

% \subsection{VTC J095517.5+690813}

% VTC J095517.5+690813 was discovered in M81 using Very Large Array data by \citep{2019MNRAS.489.1181A}. It rose from non-detections, doubling in less than 112 days. It is located within a star-forming region in M81, 30\,kpc offset from the centre. Since observations are in a single band, the spectral index isn't very constraiining. However, the 6 Ghz luminosity of $\sim10^{24}\:\mathrm{erg\:s^{-1}\:Hz^{-1}}$

% \subsection{J095552.5+694045.4}

% J095552.5+694045.4 was discovered in the central kiloparsec of the star-forming galaxy M82 using VLA observations by \citet{2010MNRAS.404L.109M}. The transient brightened by a factor of approximately 5 in less than a week. At the time of the last observation, it had been detectable for nearly 300 days with no signs of fading. The spectral index remained steady at $-0.7$ throughout the 150-day monitoring period, consistent with optically thin synchrotron emission. The 5\,GHz luminosity of the source is $\sim10^{25}\:\mathrm{erg\:s^{-1}\:Hz^{-1}}$, which could be consistent with the late-time Netwonian evolution of a short GRB, such as the radio afterglow associated with GW170817 \citep{2022ApJ...938...12B}.

2023-05-04 & $3.87^{+1.04}_{-0.95}$ & $1.82^{+0.80}_{-0.88}$ & $-0.87^{+0.26}_{-0.35}$ & $2.74^{+0.52}_{-0.70}$ & 3.14 \\
2023-06-08 & $4.18^{+1.05}_{-0.98}$ & $1.29^{+0.60}_{-0.52}$ & $-0.75^{+0.19}_{-0.24}$ & $2.50^{+0.37}_{-0.49}$ & 0.61 \\
2023-08-27 & $4.78^{+1.30}_{-1.13}$ & $1.25^{+0.58}_{-0.50}$ & $-0.89^{+0.18}_{-0.23}$ & $2.79^{+0.37}_{-0.46}$ & 0.23 \\
2023-11-29 & $4.10^{+0.84}_{-0.83}$ & $1.10^{+0.35}_{-0.31}$ & $-0.81^{+0.17}_{-0.18}$ & $2.62^{+0.33}_{-0.37}$ & 0.07 \\
2024-03-10 & $3.31^{+0.68}_{-0.58}$ & $0.74^{+0.14}_{-0.13}$ & $-0.71^{+0.12}_{-0.13}$ & $2.42^{+0.23}_{-0.27}$ & 0.72 \\
2024-06-24 & $3.29^{+0.72}_{-0.68}$ & $1.04^{+0.18}_{-0.18}$ & $-0.82^{+0.16}_{-0.15}$ & $2.64^{+0.32}_{-0.30}$ & 0.2  \\
2024-09-24 & $3.33^{+0.72}_{-0.66}$ & $0.89^{+0.33}_{-0.25}$ & $-0.78^{+0.13}_{-0.16}$ & $2.57^{+0.26}_{-0.31}$ & 0.08 \\
2024-12-26 & $3.11^{+0.62}_{-0.62}$ & $1.30^{+0.23}_{-0.19}$ & $-1.04^{+0.16}_{-0.16}$ & $3.08^{+0.33}_{-0.32}$ & 0.42 \\
2025-03-20 & $3.89^{+0.88}_{-0.81}$ & $0.95^{+0.32}_{-0.28}$ & $-1.12^{+0.16}_{-0.19}$ & $3.23^{+0.31}_{-0.37}$ & 0.17 


\begin{center}
\setlength{\tabcolsep}{2pt}
\begin{longtable*}{l|l|l|l|l|l|l|l}
\caption{Physical outflow parameters for ASKAP J0055–2558 derived from equipartition modeling of the radio spectra, assuming different outflow geometries. For each epoch, we list the equipartition radius ($R_{\rm eq}$), energy ($E_{\rm eq}$), outflow velocity ($\beta = v/c$), ejected mass ($M_{\rm ej}$), magnetic field strength ($B$), and ambient number density ($n_0$). Uncertainties represent 1$\sigma$ credible intervals derived from MCMC fitting of the SBPL spectral parameters shown in Figure~\ref{fig:SBPL_params}.}
\label{Table:Outflow_params} \\
\hline
\hline
Geometry &
\begin{tabular}[c]{@{}l@{}} Date \\ UTC \end{tabular} &
\begin{tabular}[c]{@{}l@{}}Req \\ (cm)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}$E_{\rm eq}$ \\ (erg)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}$\beta$\\  (c)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}$M_{\rm ej}$\\  (g)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}B\\  (G)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}$n_0$\\  $({\rm cm}^{-3})$\end{tabular} \\ 
 \hline
Spherical 
& 2023-05-04 & $4.67^{+0.30}_{-5.11} \times 10^{17}$ & $5.43^{+35.77}_{-4.10} \times 10^{50}$ & $2.88^{+0.13}_{-1.71} \times 10^{-1}$ & $1.45^{+10.66}_{-1.31} \times 10^{31}$ & $2.07^{+4.11}_{-0.31} \times 10^{-1}$ & $6.01^{+2.73}_{-5.46} \times 10^{-2}$ \\
& 2023-06-08 & $6.75^{+1.30}_{-5.93} \times 10^{17}$ & $4.62^{+10.98}_{-2.73} \times 10^{50}$ & $3.52^{+0.47}_{-1.53} \times 10^{-1}$ & $8.28^{+29.03}_{-6.64} \times 10^{30}$ & $1.12^{+1.65}_{-0.30} \times 10^{-1}$ & $4.02^{+0.15}_{-3.66} \times 10^{-2}$ \\
 & 2023-08-27 & $7.69^{+1.45}_{-3.03} \times 10^{17}$ & $9.72^{+9.79}_{-6.56} \times 10^{50}$ & $3.47^{+0.46}_{-0.79} \times 10^{-1}$ & $1.79^{+2.98}_{-1.41} \times 10^{31}$ & $1.31^{+1.20}_{-0.82} \times 10^{-1}$ & $2.61^{+0.60}_{-0.65} \times 10^{-2}$ \\
 & 2023-11-29 & $8.43^{+1.03}_{-1.59} \times 10^{17}$ & $5.78^{+5.87}_{-3.21} \times 10^{50}$ & $3.33^{+0.28}_{-0.39} \times 10^{-1}$ & $1.16^{+1.63}_{-0.75} \times 10^{31}$ & $8.93^{+6.25}_{-4.01} \times 10^{-2}$ & $2.39^{+0.16}_{-0.36} \times 10^{-2}$ \\
 & 2024-03-10 & $1.09^{+0.05}_{-0.07} \times 10^{18}$ & $4.12^{+3.15}_{-1.94} \times 10^{50}$ & $3.60^{+0.11}_{-0.15} \times 10^{-1}$ & $7.09^{+6.22}_{-3.64} \times 10^{30}$ & $5.22^{+2.07}_{-1.38} \times 10^{-2}$ & $1.50^{+0.00}_{-0.13} \times 10^{-2}$ \\
 & 2024-06-24 & $8.07^{+0.09}_{-0.22} \times 10^{17}$ & $4.87^{+5.62}_{-2.59} \times 10^{50}$ & $2.67^{+0.02}_{-0.05} \times 10^{-1}$ & $1.52^{+1.81}_{-0.84} \times 10^{31}$ & $8.75^{+4.13}_{-2.80} \times 10^{-2}$ & $2.24^{+0.31}_{-0.13} \times 10^{-2}$ \\
 & 2024-09-24 & $9.25^{+1.57}_{-1.78} \times 10^{17}$ & $4.99^{+3.03}_{-2.39} \times 10^{50}$ & $2.74^{+0.35}_{-0.36} \times 10^{-1}$ & $1.47^{+1.65}_{-0.88} \times 10^{31}$ & $7.23^{+4.72}_{-3.01} \times 10^{-2}$ & $1.83^{+0.53}_{-0.38} \times 10^{-2}$ \\
 & 2024-12-26 & $6.74^{+0.11}_{-0.04} \times 10^{17}$ & $8.44^{+9.93}_{-4.73} \times 10^{50}$ & $2.01^{+0.03}_{-0.01} \times 10^{-1}$ & $4.66^{+5.75}_{-2.60} \times 10^{31}$ & $1.48^{+0.74}_{-0.48} \times 10^{-1}$ & $2.12^{+0.33}_{-0.36} \times 10^{-2}$ \\
 & 2025-03-20 & $1.07^{+0.14}_{-0.18} \times 10^{18}$ & $2.05^{+1.39}_{-1.01} \times 10^{51}$ & $2.70^{+0.27}_{-0.32} \times 10^{-1}$ & $6.27^{+6.71}_{-3.73} \times 10^{31}$ & $1.15^{+0.68}_{-0.50} \times 10^{-1}$ & $8.54^{+1.54}_{-1.17} \times 10^{-3}$ \\  \hline
Conical (5°) 
& 2023-05-04 & $3.43^{+0.06}_{-3.43} \times 10^{18}$ & $1.72^{+20.48}_{-1.47} \times 10^{52}$ & $7.49^{+0.03}_{-1.07} \times 10^{-1}$ & $6.83^{+82.04}_{-6.06} \times 10^{31}$ & $3.51^{+9.20}_{-1.03} \times 10^{-2}$ & $3.22^{+1.97}_{-2.81} \times 10^{-4}$ \\
& 2023-06-08 & $4.89^{+0.81}_{-4.02} \times 10^{18}$ & $1.24^{+4.74}_{-0.88} \times 10^{52}$  & $7.97^{+0.31}_{-0.80} \times 10^{-1}$ & $4.33^{+18.31}_{-3.29} \times 10^{31}$ & $1.78^{+3.24}_{-0.22} \times 10^{-2}$ & $2.39^{+0.56}_{-2.13} \times 10^{-4}$ \\
 & 2023-08-27 & $5.65^{+0.98}_{-1.98} \times 10^{18}$ & $3.02^{+4.44}_{-2.33} \times 10^{52}$ & $7.96^{+0.33}_{-0.44} \times 10^{-1}$ & $1.06^{+1.79}_{-0.84} \times 10^{32}$ & $2.21^{+2.36}_{-1.48} \times 10^{-2}$ & $1.42^{+0.11}_{-0.08} \times 10^{-4}$ \\
 & 2023-11-29 & $6.11^{+0.65}_{-1.00} \times 10^{18}$ & $1.57^{+2.27}_{-1.02} \times 10^{52}$ & $7.84^{+0.20}_{-0.25} \times 10^{-1}$ & $5.70^{+8.96}_{-3.80} \times 10^{31}$ & $1.43^{+1.18}_{-0.71} \times 10^{-2}$ & $1.41^{+0.08}_{-0.02} \times 10^{-4}$ \\
 & 2024-03-10 & $7.83^{+0.28}_{-0.42} \times 10^{18}$ & $9.92^{+10.13}_{-5.44}\times 10^{51}$ & $8.01^{+0.06}_{-0.08} \times 10^{-1}$ & $3.44^{+3.61}_{-1.92} \times 10^{31}$ & $8.00^{+3.74}_{-2.44} \times 10^{-3}$ & $9.56^{+0.77}_{-0.06} \times 10^{-5}$ \\
 & 2024-06-24 & $5.85^{+0.03}_{-0.06} \times 10^{18}$ & $1.34^{+2.11}_{-0.81} \times 10^{52}$ & $7.26^{+0.01}_{-0.02} \times 10^{-1}$ & $5.65^{+8.87}_{-3.44} \times 10^{31}$ & $1.41^{+0.80}_{-0.51} \times 10^{-2}$ & $1.32^{+0.31}_{-0.24} \times 10^{-4}$ \\
 & 2024-09-24 & $6.69^{+1.06}_{-1.15} \times 10^{18}$ & $1.32^{+1.14}_{-0.75} \times 10^{52}$ & $7.32^{+0.35}_{-0.30} \times 10^{-1}$ & $5.48^{+5.78}_{-3.30} \times 10^{31}$ & $1.15^{+0.85}_{-0.52} \times 10^{-2}$ & $1.10^{+0.19}_{-0.12} \times 10^{-4}$ \\
 & 2024-12-26 & $4.99^{+0.00}_{-0.11} \times 10^{18}$ & $2.89^{+4.69}_{-1.83} \times 10^{52}$ & $6.50^{+0.00}_{-0.05} \times 10^{-1}$ & $1.52^{+2.47}_{-0.96} \times 10^{32}$ & $2.59^{+1.57}_{-0.95} \times 10^{-2}$ & $1.08^{+0.27}_{-0.34} \times 10^{-4}$ \\
 & 2025-03-20 & $7.98^{+0.96}_{-1.22} \times 10^{18}$ & $7.57^{+7.07}_{-4.38} \times 10^{52}$ & $7.34^{+0.26}_{-0.27} \times 10^{-1}$ & $3.13^{+3.37}_{-1.90} \times 10^{32}$ & $2.07^{+1.40}_{-0.97} \times 10^{-2}$ & $4.15^{+0.32}_{-0.11} \times 10^{-5}$ \\ \hline
Conical (15°) 
& 2023-05-04 & $1.36^{+0.05}_{-1.41} \times 10^{18}$ & $4.39^{+41.49}_{-3.59} \times 10^{51}$ & $5.42^{+0.09}_{-1.65} \times 10^{-1}$ & $3.32^{+32.60}_{-2.97} \times 10^{31}$ & $7.09^{+16.67}_{-1.70} \times 10^{-2}$ & $2.55^{+1.41}_{-2.26} \times 10^{-3}$ \\
& 2023-06-08 & $1.95^{+0.34}_{-1.65} \times 10^{18}$ & $3.37^{+10.76}_{-2.25} \times 10^{51}$ & $6.11^{+0.47}_{-1.32} \times 10^{-1}$ & $2.01^{+7.87}_{-1.56} \times 10^{31}$ & $3.68^{+6.18}_{-0.65} \times 10^{-2}$ & $1.82^{+0.29}_{-1.63} \times 10^{-3}$ \\
& 2023-08-27 & $2.25^{+0.40}_{-0.82} \times 10^{18}$ & $7.76^{+9.89}_{-5.72} \times 10^{51}$ & $6.08^{+0.48}_{-0.72} \times 10^{-1}$ & $4.67^{+7.85}_{-3.69} \times 10^{31}$ & $4.47^{+4.50}_{-2.93} \times 10^{-2}$ & $1.12^{+0.15}_{-0.16} \times 10^{-3}$ \\
& 2023-11-29 & $2.44^{+0.28}_{-0.42} \times 10^{18}$ & $4.26^{+5.39}_{-2.61} \times 10^{51}$ & $5.92^{+0.29}_{-0.38} \times 10^{-1}$ & $2.71^{+4.08}_{-1.78} \times 10^{31}$ & $2.95^{+2.29}_{-1.41} \times 10^{-2}$ & $1.07^{+0.01}_{-0.08} \times 10^{-3}$ \\
& 2024-03-10 & $3.14^{+0.13}_{-0.19} \times 10^{18}$ & $2.82^{+2.58}_{-1.46} \times 10^{51}$ & $6.18^{+0.10}_{-0.14} \times 10^{-1}$ & $1.64^{+1.61}_{-0.89} \times 10^{31}$ & $1.68^{+0.74}_{-0.49} \times 10^{-2}$ & $7.06^{+0.34}_{-0.23} \times 10^{-4}$ \\
& 2024-06-24 & $2.34^{+0.00}_{-0.04} \times 10^{18}$ & $3.61^{+5.05}_{-2.09} \times 10^{51}$ & $5.14^{+0.00}_{-0.04} \times 10^{-1}$ & $3.04^{+4.27}_{-1.78} \times 10^{31}$ & $2.90^{+1.54}_{-1.00} \times 10^{-2}$ & $1.00^{+0.20}_{-0.13} \times 10^{-3}$ \\
& 2024-09-24 & $2.68^{+0.44}_{-0.48} \times 10^{18}$ & $3.62^{+2.74}_{-1.93} \times 10^{51}$ & $5.22^{+0.44}_{-0.41} \times 10^{-1}$ & $2.95^{+3.24}_{-1.77} \times 10^{31}$ & $2.38^{+1.68}_{-1.04} \times 10^{-2}$ & $8.29^{+1.80}_{-1.22} \times 10^{-4}$ \\
& 2024-12-26 & $1.98^{+0.01}_{-0.03} \times 10^{18}$ & $7.15^{+10.26}_{-4.34}\times 10^{51}$ & $4.24^{+0.01}_{-0.04} \times 10^{-1}$ & $8.84^{+12.84}_{-5.30}\times 10^{31}$ & $5.17^{+2.91}_{-1.81} \times 10^{-2}$ & $8.70^{+1.84}_{-2.20} \times 10^{-4}$ \\
& 2025-03-20 & $3.15^{+0.39}_{-0.50} \times 10^{18}$ & $1.82^{+1.50}_{-0.99} \times 10^{52}$ & $5.21^{+0.33}_{-0.37} \times 10^{-1}$ & $1.49^{+1.62}_{-0.90} \times 10^{32}$ & $4.08^{+2.63}_{-1.86} \times 10^{-2}$ & $3.41^{+0.40}_{-0.25} \times 10^{-4}$ \\ \hline
Conical (30°) 
& 2023-05-04  & $7.62^{+0.36}_{-8.07} \times 10^{17}$ & $1.85^{+15.12}_{-1.47} \times 10^{51}$ & $3.98^{+0.12}_{-1.79} \times 10^{-1}$ & $2.60^{+22.67}_{-2.35} \times 10^{31}$ & $1.10^{+2.42}_{-0.22} \times 10^{-1}$ & $9.39^{+4.85}_{-8.42} \times 10^{-3}$ \\
& 2023-06-08 & $1.09^{+0.20}_{-0.94} \times 10^{18}$ & $1.48^{+4.21}_{-0.95} \times 10^{51}$ & $4.69^{+0.50}_{-1.53} \times 10^{-1}$ & $1.50^{+5.72}_{-1.19} \times 10^{31}$ & $5.82^{+9.26}_{-1.25} \times 10^{-2}$ & $6.52^{+0.73}_{-5.89} \times 10^{-3}$ \\
& 2023-08-27 & $1.25^{+0.23}_{-0.47} \times 10^{18}$ & $3.29^{+3.82}_{-2.35} \times 10^{51}$ & $4.64^{+0.50}_{-0.80} \times 10^{-1}$ & $3.40^{+5.81}_{-2.69} \times 10^{31}$ & $6.97^{+6.76}_{-4.48} \times 10^{-2}$ & $4.10^{+0.71}_{-0.77} \times 10^{-3}$ \\
& 2023-11-29 & $1.37^{+0.16}_{-0.25} \times 10^{18}$ & $1.87^{+2.16}_{-1.10} \times 10^{51}$ & $4.48^{+0.30}_{-0.41} \times 10^{-1}$ & $2.07^{+3.07}_{-1.36} \times 10^{31}$ & $4.66^{+3.46}_{-2.17} \times 10^{-2}$ & $3.87^{+0.08}_{-0.40} \times 10^{-3}$ \\
& 2024-03-10 & $1.77^{+0.08}_{-0.11} \times 10^{18}$ & $1.27^{+1.09}_{-0.64} \times 10^{51}$ & $4.76^{+0.11}_{-0.15} \times 10^{-1}$ & $1.25^{+1.18}_{-0.66} \times 10^{31}$ & $2.68^{+1.13}_{-0.75} \times 10^{-2}$ & $2.49^{+0.07}_{-0.14} \times 10^{-3}$ \\
& 2024-06-24 & $1.31^{+0.01}_{-0.03} \times 10^{18}$ & $1.58^{+2.04}_{-0.88} \times 10^{51}$ & $3.72^{+0.01}_{-0.05} \times 10^{-1}$ & $2.54^{+3.33}_{-1.45} \times 10^{31}$ & $4.57^{+2.32}_{-1.53} \times 10^{-2}$ & $3.62^{+0.63}_{-0.36} \times 10^{-3}$ \\
& 2024-09-24 & $1.50^{+0.25}_{-0.28} \times 10^{18}$ & $1.60^{+1.11}_{-0.82} \times 10^{51}$ & $3.80^{+0.42}_{-0.41} \times 10^{-1}$ & $2.46^{+2.79}_{-1.48} \times 10^{31}$ & $3.76^{+2.57}_{-1.62} \times 10^{-2}$ & $2.97^{+0.73}_{-0.51} \times 10^{-3}$ \\
& 2024-12-26 & $1.10^{+0.01}_{-0.01} \times 10^{18}$ & $2.96^{+3.92}_{-1.74} \times 10^{51}$ & $2.91^{+0.02}_{-0.02} \times 10^{-1}$ & $7.77^{+10.56}_{-4.52}\times 10^{31}$ & $7.99^{+4.29}_{-2.71} \times 10^{-2}$ & $3.25^{+0.61}_{-0.71} \times 10^{-3}$ \\
& 2025-03-20 & $1.75^{+0.22}_{-0.29} \times 10^{18}$ & $7.38^{+5.64}_{-3.87} \times 10^{51}$ & $3.77^{+0.32}_{-0.37} \times 10^{-1}$ & $1.15^{+1.27}_{-0.70} \times 10^{32}$ & $6.26^{+3.90}_{-2.79} \times 10^{-2}$ & $1.29^{+0.18}_{-0.13} \times 10^{-3}$ \\
 \hline
\end{longtable*}
\end{center}


\begin{center}
% \setlength{\tabcolsep}{0.2pt}
\label{Table:Corrected_R_E}
\begin{longtable*}{lllllllll}
\caption{Equipartition-corrected outflow radius ($R$) and energy ($E$) for ASKAP J0055–2558 across multiple epochs, computed for different outflow geometries: spherical, and conical with opening angles of $5^\circ$, $15^\circ$, and $30^\circ$. All values are derived assuming different combinations of $\varepsilon_e$ and $\varepsilon_B$. }\\
\hline
\hline
\multicolumn{1}{c}{} &
  \multicolumn{2}{c}{Spherical} &
  \multicolumn{2}{c}{Conical($5^\circ$)} &
  \multicolumn{2}{c}{Conical($15^\circ$)} &
  \multicolumn{2}{c}{Conical($30^\circ$)} \\ \hline
Epoch &
  $R$ ($10^{17}$ cm) &
  $E$ ($10^{51}$ erg) &
  $R$ ($10^{17}$ cm) &
  $E$ ($10^{51}$ erg) &
  $R$ ($10^{17}$ cm) &
  $E$ ($10^{51}$ erg) &
  $R$ ($10^{17}$ cm) &
  $E$ ($10^{51}$ erg) \\ \hline
\multicolumn{9}{c}{$\varepsilon_e$ = 0.0005; $\varepsilon_B$ = 0.001} \\ \hline

2023-05-04 & $5.04^{+0.32}_{-5.51}$ & $0.67^{+4.39}_{-0.50}$ & $37.08^{+0.63}_{-37.03}$ & $21.11^{+251.31}_{-17.99}$ & $14.73^{+0.53}_{-15.25}$ & $5.38^{+50.92}_{-4.41}$ & $8.23^{+0.39}_{-8.71}$ & $2.27^{+18.55}_{-1.81}$ \\ 2023-06-08 & $7.28^{+1.40}_{-6.41}$ & $0.57^{+1.35}_{-0.34}$ & $52.73^{+8.75}_{-43.38}$ & $15.17^{+58.16}_{-10.76}$ & $21.07^{+3.72}_{-17.81}$ & $4.13^{+13.21}_{-2.76}$ & $11.82^{+2.17}_{-10.15}$ & $1.82^{+5.16}_{-1.16}$ \\
2023-08-27 &
  $8.30^{+1.56}_{-3.27}$ &
  $1.19^{+1.20}_{-0.80}$ &
  $60.96^{+10.54}_{-21.33}$ &
  $37.03^{+54.44}_{-28.58}$ &
  $24.23^{+4.34}_{-8.90}$ &
  $9.52^{+12.14}_{-7.02}$ &
  $13.54^{+2.48}_{-5.12}$ &
  $4.04^{+4.69}_{-2.88}$ \\
2023-11-29 &
  $9.10^{+1.11}_{-1.71}$ &
  $0.71^{+0.72}_{-0.39}$ &
  $65.99^{+7.03}_{-10.81}$ &
  $19.30^{+27.89}_{-12.47}$ &
  $26.36^{+2.97}_{-4.57}$ &
  $5.23^{+6.61}_{-3.20}$ &
  $14.77^{+1.72}_{-2.65}$ &
  $2.29^{+2.65}_{-1.35}$ \\
2024-03-10 &
  $11.79^{+0.55}_{-0.81}$ &
  $0.51^{+0.39}_{-0.24}$ &
  $84.57^{+2.98}_{-4.52}$ &
  $12.17^{+12.43}_{-6.68}$ &
  $33.93^{+1.35}_{-2.01}$ &
  $3.46^{+3.17}_{-1.80}$ &
  $19.07^{+0.82}_{-1.20}$ &
  $1.56^{+1.33}_{-0.78}$ \\
2024-06-24 &
  $8.71^{+0.10}_{-0.23}$ &
  $0.60^{+0.69}_{-0.32}$ &
  $63.20^{+0.30}_{-0.69}$ &
  $16.41^{+25.86}_{-9.95}$ &
  $25.23^{+0.04}_{-0.44}$ &
  $4.43^{+6.20}_{-2.56}$ &
  $14.14^{+0.08}_{-0.30}$ &
  $1.94^{+2.51}_{-1.08}$ \\
2024-09-24 &
  $9.99^{+1.69}_{-1.92}$ &
  $0.61^{+0.37}_{-0.29}$ &
  $72.26^{+11.44}_{-12.47}$ &
  $16.21^{+13.97}_{-9.21}$ &
  $28.89^{+4.70}_{-5.21}$ &
  $4.44^{+3.36}_{-2.37}$ &
  $16.20^{+2.68}_{-3.00}$ &
  $1.96^{+1.36}_{-1.00}$ \\
2024-12-26 &
  $7.27^{+0.12}_{-0.04}$ &
  $1.04^{+1.22}_{-0.58}$ &
  $53.86^{+0.04}_{-1.20}$ &
  $35.50^{+57.55}_{-22.49}$ &
  $21.33^{+0.13}_{-0.34}$ &
  $8.77^{+12.59}_{-5.32}$ &
  $11.89^{+0.12}_{-0.14}$ &
  $3.63^{+4.81}_{-2.14}$ \\
2025-03-20 &
  $11.55^{+1.52}_{-1.99}$ &
  $2.52^{+1.70}_{-1.24}$ &
  $86.09^{+10.39}_{-13.12}$ &
  $92.85^{+86.74}_{-53.76}$ &
  $34.01^{+4.26}_{-5.45}$ &
  $22.29^{+18.45}_{-12.18}$ &
  $18.93^{+2.42}_{-3.13}$ &
  $9.06^{+6.92}_{-4.75}$ \\ \hline
\multicolumn{9}{c}{$\varepsilon_e$ = 0.0005; $\varepsilon_B$ = 0.01} \\ \hline

2023-05-04 & $5.77^{+0.37}_{-6.31}$ & $2.07^{+13.63}_{-1.56}$ & $42.45^{+0.73}_{-42.41}$ & $65.57^{+780.48}_{-55.87}$ & $16.86^{+0.60}_{-17.47}$ & $16.72^{+158.15}_{-13.70}$ & $9.42^{+0.45}_{-9.98}$ & $7.06^{+57.61}_{-5.61}$ \\
2023-06-08 & $8.34^{+1.61}_{-7.34}$ & $1.76^{+4.18}_{-1.04}$ & $60.38^{+10.02}_{-49.67}$ & $47.11^{+180.63}_{-33.43}$ & $24.13^{+4.26}_{-20.39}$ & $12.84^{+41.02}_{-8.57}$ & $13.53^{+2.48}_{-11.63}$ & $5.65^{+16.03}_{-3.61}$ \\
2023-08-27 &
  $9.51^{+1.79}_{-3.75}$ &
  $3.71^{+3.73}_{-2.50}$ &
  $69.80^{+12.07}_{-24.42}$ &
  $115.01^{+169.08}_{-88.76}$ &
  $27.75^{+4.97}_{-10.19}$ &
  $29.56^{+37.71}_{-21.80}$ &
  $15.51^{+2.84}_{-5.87}$ &
  $12.55^{+14.56}_{-8.95}$ \\
2023-11-29 &
  $10.42^{+1.27}_{-1.96}$ &
  $2.20^{+2.24}_{-1.22}$ &
  $75.56^{+8.05}_{-12.37}$ &
  $59.94^{+86.60}_{-38.72}$ &
  $30.18^{+3.40}_{-5.23}$ &
  $16.23^{+20.53}_{-9.94}$ &
  $16.91^{+1.97}_{-3.04}$ &
  $7.12^{+8.25}_{-4.20}$ \\
2024-03-10 &
  $13.50^{+0.64}_{-0.93}$ &
  $1.57^{+1.20}_{-0.74}$ &
  $96.84^{+3.41}_{-5.17}$ &
  $37.79^{+38.60}_{-20.73}$ &
  $38.85^{+1.55}_{-2.31}$ &
  $10.74^{+9.84}_{-5.58}$ &
  $21.83^{+0.94}_{-1.38}$ &
  $4.86^{+4.14}_{-2.43}$ \\
2024-06-24 &
  $9.97^{+0.11}_{-0.27}$ &
  $1.86^{+2.14}_{-0.99}$ &
  $72.36^{+0.34}_{-0.79}$ &
  $50.98^{+80.30}_{-30.89}$ &
  $28.89^{+0.05}_{-0.50}$ &
  $13.76^{+19.25}_{-7.95}$ &
  $16.19^{+0.09}_{-0.34}$ &
  $6.02^{+7.79}_{-3.37}$ \\
2024-09-24 &
  $11.44^{+1.94}_{-2.20}$ &
  $1.90^{+1.16}_{-0.91}$ &
  $82.74^{+13.10}_{-14.28}$ &
  $50.35^{+43.40}_{-28.60}$ &
  $33.08^{+5.38}_{-5.97}$ &
  $13.78^{+10.43}_{-7.37}$ &
  $18.55^{+3.07}_{-3.44}$ &
  $6.08^{+4.22}_{-3.12}$ \\
2024-12-26 &
  $8.33^{+0.13}_{-0.05}$ &
  $3.22^{+3.78}_{-1.80}$ &
  $61.67^{+0.04}_{-1.38}$ &
  $110.26^{+178.73}_{-69.84}$ &
  $24.43^{+0.15}_{-0.39}$ &
  $27.25^{+39.11}_{-16.52}$ &
  $13.62^{+0.14}_{-0.16}$ &
  $11.28^{+14.95}_{-6.64}$ \\
2025-03-20 &
  $13.22^{+1.75}_{-2.28}$ &
  $7.82^{+5.28}_{-3.84}$ &
  $98.58^{+11.90}_{-15.02}$ &
  $288.37^{+269.39}_{-166.96}$ &
  $38.95^{+4.88}_{-6.24}$ &
  $69.23^{+57.30}_{-37.83}$ &
  $21.68^{+2.78}_{-3.58}$ &
  $28.14^{+21.48}_{-14.76}$ \\ \hline
\multicolumn{9}{c}{$\varepsilon_e$ = 0.0005; $\varepsilon_B$ = 0.1} \\ \hline
2023-05-04 & $6.61^{+0.42}_{-7.23}$ & $8.79^{+57.89}_{-6.63}$ & $48.61^{+0.83}_{-48.56}$ & $278.43^{+3314.32}_{-237.25}$ & $19.31^{+0.69}_{-20.00}$ & $71.01^{+671.57}_{-58.17}$ & $10.79^{+0.51}_{-11.42}$ & $29.99^{+244.65}_{-23.84}$ \\
2023-06-08 & $9.55^{+1.84}_{-8.40}$ & $7.47^{+17.77}_{-4.42}$ & $69.14^{+11.48}_{-56.88}$ & $200.04^{+767.05}_{-141.96}$ & $27.63^{+4.88}_{-23.35}$ & $54.51^{+174.21}_{-36.41}$ & $15.49^{+2.84}_{-13.31}$ & $24.00^{+68.09}_{-15.33}$ \\
2023-08-27 &
  $10.89^{+2.05}_{-4.29}$ &
  $15.74^{+15.84}_{-10.61}$ &
  $79.93^{+13.82}_{-27.96}$ &
  $488.40^{+718.01}_{-376.91}$ &
  $31.77^{+5.69}_{-11.67}$ &
  $125.55^{+160.12}_{-92.57}$ &
  $17.75^{+3.25}_{-6.72}$ &
  $53.28^{+61.83}_{-37.99}$ \\
2023-11-29 &
  $11.93^{+1.46}_{-2.25}$ &
  $9.36^{+9.50}_{-5.19}$ &
  $86.52^{+9.22}_{-14.17}$ &
  $254.56^{+367.77}_{-164.42}$ &
  $34.56^{+3.90}_{-5.99}$ &
  $68.94^{+87.19}_{-42.21}$ &
  $19.37^{+2.26}_{-3.48}$ &
  $30.23^{+35.01}_{-17.82}$ \\
2024-03-10 &
  $15.46^{+0.73}_{-1.06}$ &
  $6.67^{+5.10}_{-3.15}$ &
  $110.89^{+3.91}_{-5.92}$ &
  $160.47^{+163.90}_{-88.05}$ &
  $44.49^{+1.78}_{-2.64}$ &
  $45.62^{+41.78}_{-23.71}$ &
  $25.00^{+1.07}_{-1.58}$ &
  $20.63^{+17.58}_{-10.32}$ \\
2024-06-24 &
  $11.41^{+0.13}_{-0.31}$ &
  $7.89^{+9.09}_{-4.20}$ &
  $82.86^{+0.39}_{-0.91}$ &
  $216.47^{+340.99}_{-131.17}$ &
  $33.08^{+0.06}_{-0.57}$ &
  $58.42^{+81.73}_{-33.78}$ &
  $18.54^{+0.11}_{-0.39}$ &
  $25.57^{+33.08}_{-14.31}$ \\
2024-09-24 &
  $13.09^{+2.22}_{-2.52}$ &
  $8.07^{+4.91}_{-3.87}$ &
  $94.74^{+15.00}_{-16.35}$ &
  $213.80^{+184.28}_{-121.44}$ &
  $37.88^{+6.17}_{-6.83}$ &
  $58.52^{+44.30}_{-31.31}$ &
  $21.24^{+3.52}_{-3.94}$ &
  $25.84^{+17.93}_{-13.25}$ \\
2024-12-26 &
  $9.53^{+0.15}_{-0.06}$ &
  $13.66^{+16.07}_{-7.66}$ &
  $70.62^{+0.05}_{-1.58}$ &
  $468.23^{+758.98}_{-296.60}$ &
  $27.97^{+0.17}_{-0.45}$ &
  $115.73^{+166.09}_{-70.17}$ &
  $15.59^{+0.16}_{-0.19}$ &
  $47.91^{+63.48}_{-28.18}$ \\
2025-03-20 &
  $15.14^{+2.00}_{-2.61}$ &
  $33.19^{+22.44}_{-16.32}$ &
  $112.88^{+13.63}_{-17.20}$ &
  $1224.56^{+1143.98}_{-709.00}$ &
  $44.59^{+5.58}_{-7.14}$ &
  $293.97^{+243.32}_{-160.64}$ &
  $24.82^{+3.18}_{-4.10}$ &
  $119.49^{+91.24}_{-62.69}$ \\ \hline
\multicolumn{9}{c}{$\varepsilon_e$ = 0.1; $\varepsilon_B$ = 0.001} \\ \hline
2023-05-04 & $3.69^{+0.23}_{-4.04}$ & $1.46^{+9.59}_{-1.10}$ & $27.15^{+0.46}_{-27.12}$ & $46.12^{+548.95}_{-39.30}$ & $10.78^{+0.39}_{-11.17}$ & $11.76^{+111.23}_{-9.64}$ & $6.02^{+0.28}_{-6.38}$ & $4.97^{+40.52}_{-3.95}$ \\
2023-06-08 & $5.33^{+1.03}_{-4.69}$ & $1.24^{+2.94}_{-0.73}$ & $38.61^{+6.41}_{-31.77}$ & $33.13^{+127.05}_{-23.51}$ & $15.43^{+2.73}_{-13.04}$ & $9.03^{+28.85}_{-6.03}$ & $8.65^{+1.59}_{-7.43}$ & $3.98^{+11.28}_{-2.54}$ \\
2023-08-27 &
  $6.08^{+1.15}_{-2.40}$ &
  $2.61^{+2.62}_{-1.76}$ &
  $44.64^{+7.72}_{-15.62}$ &
  $80.89^{+118.92}_{-62.43}$ &
  $17.74^{+3.18}_{-6.52}$ &
  $20.79^{+26.52}_{-15.33}$ &
  $9.92^{+1.81}_{-3.75}$ &
  $8.82^{+10.24}_{-6.29}$ \\
2023-11-29 &
  $6.66^{+0.81}_{-1.25}$ &
  $1.55^{+1.57}_{-0.86}$ &
  $48.32^{+5.15}_{-7.91}$ &
  $42.16^{+60.91}_{-27.23}$ &
  $19.30^{+2.18}_{-3.35}$ &
  $11.42^{+14.44}_{-6.99}$ &
  $10.82^{+1.26}_{-1.94}$ &
  $5.01^{+5.80}_{-2.95}$ \\
2024-03-10 &
  $8.63^{+0.41}_{-0.59}$ &
  $1.10^{+0.85}_{-0.52}$ &
  $61.93^{+2.18}_{-3.31}$ &
  $26.58^{+27.15}_{-14.58}$ &
  $24.84^{+0.99}_{-1.48}$ &
  $7.56^{+6.92}_{-3.93}$ &
  $13.96^{+0.60}_{-0.88}$ &
  $3.42^{+2.91}_{-1.71}$ \\
2024-06-24 &
  $6.37^{+0.07}_{-0.17}$ &
  $1.31^{+1.51}_{-0.69}$ &
  $46.27^{+0.22}_{-0.51}$ &
  $35.85^{+56.48}_{-21.73}$ &
  $18.48^{+0.03}_{-0.32}$ &
  $9.68^{+13.54}_{-5.59}$ &
  $10.35^{+0.06}_{-0.22}$ &
  $4.23^{+5.48}_{-2.37}$ \\
2024-09-24 &
  $7.31^{+1.24}_{-1.41}$ &
  $1.34^{+0.81}_{-0.64}$ &
  $52.91^{+8.38}_{-9.13}$ &
  $35.41^{+30.52}_{-20.11}$ &
  $21.15^{+3.44}_{-3.82}$ &
  $9.69^{+7.34}_{-5.19}$ &
  $11.86^{+1.96}_{-2.20}$ &
  $4.28^{+2.97}_{-2.19}$ \\
2024-12-26 &
  $5.32^{+0.09}_{-0.03}$ &
  $2.26^{+2.66}_{-1.27}$ &
  $39.44^{+0.03}_{-0.88}$ &
  $77.55^{+125.71}_{-49.13}$ &
  $15.62^{+0.09}_{-0.25}$ &
  $19.17^{+27.51}_{-11.62}$ &
  $8.71^{+0.09}_{-0.10}$ &
  $7.94^{+10.51}_{-4.67}$ \\
2025-03-20 &
  $8.45^{+1.12}_{-1.46}$ &
  $5.50^{+3.72}_{-2.70}$ &
  $63.04^{+7.61}_{-9.61}$ &
  $202.82^{+189.48}_{-117.43}$ &
  $24.90^{+3.12}_{-3.99}$ &
  $48.69^{+40.30}_{-26.61}$ &
  $13.86^{+1.78}_{-2.29}$ &
  $19.79^{+15.11}_{-10.38}$ \\ \hline
\multicolumn{9}{c}{$\varepsilon_e$ = 0.1; $\varepsilon_B$ = 0.01} \\ \hline
2023-05-04 & $4.23^{+0.27}_{-4.62}$ & $0.70^{+4.63}_{-0.53}$ & $31.09^{+0.53}_{-31.05}$ & $22.28^{+265.25}_{-18.99}$ & $12.35^{+0.44}_{-12.79}$ & $5.68^{+53.75}_{-4.66}$ & $6.90^{+0.33}_{-7.31}$ & $2.40^{+19.58}_{-1.91}$ \\
2023-06-08 & $6.10^{+1.18}_{-5.37}$ & $0.60^{+1.42}_{-0.35}$ & $44.21^{+7.34}_{-36.37}$ & $16.01^{+61.39}_{-11.36}$ & $17.67^{+3.12}_{-14.93}$ & $4.36^{+13.94}_{-2.91}$ & $9.91^{+1.82}_{-8.51}$ & $1.92^{+5.45}_{-1.23}$ \\
2023-08-27 &
  $6.96^{+1.31}_{-2.74}$ &
  $1.26^{+1.27}_{-0.85}$ &
  $51.11^{+8.84}_{-17.88}$ &
  $39.09^{+57.46}_{-30.16}$ &
  $20.32^{+3.64}_{-7.46}$ &
  $10.05^{+12.81}_{-7.41}$ &
  $11.35^{+2.08}_{-4.29}$ &
  $4.26^{+4.95}_{-3.04}$ \\
2023-11-29 &
  $7.63^{+0.93}_{-1.44}$ &
  $0.75^{+0.76}_{-0.42}$ &
  $55.33^{+5.90}_{-9.06}$ &
  $20.37^{+29.43}_{-13.16}$ &
  $22.10^{+2.49}_{-3.83}$ &
  $5.52^{+6.98}_{-3.38}$ &
  $12.38^{+1.44}_{-2.22}$ &
  $2.42^{+2.80}_{-1.43}$ \\
2024-03-10 &
  $9.89^{+0.47}_{-0.68}$ &
  $0.53^{+0.41}_{-0.25}$ &
  $70.91^{+2.50}_{-3.79}$ &
  $12.84^{+13.12}_{-7.05}$ &
  $28.45^{+1.14}_{-1.69}$ &
  $3.65^{+3.34}_{-1.90}$ &
  $15.99^{+0.69}_{-1.01}$ &
  $1.65^{+1.41}_{-0.83}$ \\
2024-06-24 &
  $7.30^{+0.08}_{-0.20}$ &
  $0.63^{+0.73}_{-0.34}$ &
  $52.98^{+0.25}_{-0.58}$ &
  $17.32^{+27.29}_{-10.50}$ &
  $21.16^{+0.04}_{-0.37}$ &
  $4.68^{+6.54}_{-2.70}$ &
  $11.85^{+0.07}_{-0.25}$ &
  $2.05^{+2.65}_{-1.15}$ \\
2024-09-24 &
  $8.37^{+1.42}_{-1.61}$ &
  $0.65^{+0.39}_{-0.31}$ &
  $60.58^{+9.59}_{-10.45}$ &
  $17.11^{+14.75}_{-9.72}$ &
  $24.22^{+3.94}_{-4.37}$ &
  $4.68^{+3.55}_{-2.51}$ &
  $13.58^{+2.25}_{-2.52}$ &
  $2.07^{+1.43}_{-1.06}$ \\
2024-12-26 &
  $6.10^{+0.10}_{-0.04}$ &
  $1.09^{+1.29}_{-0.61}$ &
  $45.16^{+0.03}_{-1.01}$ &
  $37.47^{+60.74}_{-23.74}$ &
  $17.89^{+0.11}_{-0.29}$ &
  $9.26^{+13.29}_{-5.62}$ &
  $9.97^{+0.10}_{-0.12}$ &
  $3.83^{+5.08}_{-2.26}$ \\
2025-03-20 &
  $9.68^{+1.28}_{-1.67}$ &
  $2.66^{+1.80}_{-1.31}$ &
  $72.18^{+8.71}_{-11.00}$ &
  $98.00^{+91.56}_{-56.74}$ &
  $28.52^{+3.57}_{-4.57}$ &
  $23.53^{+19.47}_{-12.86}$ &
  $15.87^{+2.03}_{-2.62}$ &
  $9.56^{+7.30}_{-5.02}$ \\ \hline
\multicolumn{9}{c}{$\varepsilon_e$ = 0.1; $\varepsilon_B$ = 0.1} \\ \hline
2023-05-04 & $4.84^{+0.31}_{-5.29}$ & $0.57^{+3.74}_{-0.43}$ & $35.59^{+0.61}_{-35.56}$ & $17.98^{+213.97}_{-15.32}$ & $14.14^{+0.50}_{-14.64}$ & $4.58^{+43.36}_{-3.76}$ & $7.90^{+0.37}_{-8.37}$ & $1.94^{+15.79}_{-1.54}$ \\
2023-06-08 & $6.99^{+1.35}_{-6.15}$ & $0.48^{+1.15}_{-0.29}$ & $50.63^{+8.41}_{-41.65}$ & $12.91^{+49.52}_{-9.16}$ & $20.23^{+3.58}_{-17.10}$ & $3.52^{+11.25}_{-2.35}$ & $11.34^{+2.08}_{-9.75}$ & $1.55^{+4.40}_{-0.99}$ \\
2023-08-27 &
  $7.97^{+1.50}_{-3.14}$ &
  $1.02^{+1.02}_{-0.69}$ &
  $58.53^{+10.12}_{-20.48}$ &
  $31.53^{+46.35}_{-24.33}$ &
  $23.27^{+4.17}_{-8.54}$ &
  $8.11^{+10.34}_{-5.98}$ &
  $13.00^{+2.38}_{-4.92}$ &
  $3.44^{+3.99}_{-2.45}$ \\
2023-11-29 &
  $8.73^{+1.07}_{-1.64}$ &
  $0.60^{+0.61}_{-0.34}$ &
  $63.35^{+6.75}_{-10.37}$ &
  $16.43^{+23.74}_{-10.62}$ &
  $25.30^{+2.85}_{-4.39}$ &
  $4.45^{+5.63}_{-2.73}$ &
  $14.18^{+1.65}_{-2.55}$ &
  $1.95^{+2.26}_{-1.15}$ \\
2024-03-10 &
  $11.32^{+0.53}_{-0.78}$ &
  $0.43^{+0.33}_{-0.20}$ &
  $81.19^{+2.86}_{-4.33}$ &
  $10.36^{+10.58}_{-5.68}$ &
  $32.57^{+1.30}_{-1.93}$ &
  $2.95^{+2.70}_{-1.53}$ &
  $18.31^{+0.78}_{-1.16}$ &
  $1.33^{+1.13}_{-0.67}$ \\
2024-06-24 &
  $8.36^{+0.10}_{-0.23}$ &
  $0.51^{+0.59}_{-0.27}$ &
  $60.67^{+0.29}_{-0.67}$ &
  $13.98^{+22.01}_{-8.47}$ &
  $24.23^{+0.04}_{-0.42}$ &
  $3.77^{+5.28}_{-2.18}$ &
  $13.57^{+0.08}_{-0.29}$ &
  $1.65^{+2.14}_{-0.92}$ \\
2024-09-24 &
  $9.59^{+1.63}_{-1.85}$ &
  $0.52^{+0.32}_{-0.25}$ &
  $69.37^{+10.98}_{-11.97}$ &
  $13.80^{+11.90}_{-7.84}$ &
  $27.74^{+4.51}_{-5.00}$ &
  $3.78^{+2.86}_{-2.02}$ &
  $15.55^{+2.57}_{-2.88}$ &
  $1.67^{+1.16}_{-0.86}$ \\
2024-12-26 &
  $6.98^{+0.11}_{-0.04}$ &
  $0.88^{+1.04}_{-0.49}$ &
  $51.71^{+0.04}_{-1.15}$ &
  $30.23^{+49.00}_{-19.15}$ &
  $20.48^{+0.12}_{-0.33}$ &
  $7.47^{+10.72}_{-4.53}$ &
  $11.42^{+0.12}_{-0.14}$ &
  $3.09^{+4.10}_{-1.82}$ \\
2025-03-20 &
  $11.08^{+1.46}_{-1.91}$ &
  $2.14^{+1.45}_{-1.05}$ &
  $82.65^{+9.98}_{-12.59}$ &
  $79.06^{+73.86}_{-45.77}$ &
  $32.65^{+4.09}_{-5.23}$ &
  $18.98^{+15.71}_{-10.37}$ &
  $18.17^{+2.33}_{-3.00}$ &
  $7.71^{+5.89}_{-4.05}$ \\ \hline
\end{longtable*}
\end{center}


The 3$\sigma$ upper limits on the flux in the 0.2--2, 2--12 and 0.2--12\,keV ranges are $1.1\times10^{-13}$, $2.9\times10^{-13}$ and $1.7\times10^{-13}\rm\,erg\,cm^{-2}\,s^{-1}$, respectively.


% Rad

% synchrotron emission in extragalactic sources. Other synchrotron transients
% limitations to discovery of extragalactic sources

% For instance, the two clases of transients that we believe ASKAP J0055–2558 may belong to one of two candidate classes of transients revealed by these new survey capabilities: a tidal disruption event (TDE) involving an intermediate-mass black hole (IMBH), or the orphan afterglow of a relativistic transient observed off-axis.

% This serves as an example of late-time radio emission discovery from an extragalactic transient whose prompt emission may have been missed.

%Deeper imaging is necessary to follow this flux further out and to see if there's something at the source position.


% We note that these values may represent an upper limit, as they are derived assuming the minimum source size corresponding to one of the earliest epochs and a spherical geometry. The actual source size is expected to be larger at later times and for more collimated outflow geometries, which would reduce the magnitude of scintillation-induced variability.





% \section{Results}
% \label{sec:results}
% % \setlength{\columnsep}{1pt}
% This section will include all the results from the multi-wavelength follow-up for this source.





% % htbp!


% \subsubsection{Spectroscopy}
% spectra - redshift, SFR and dust
% SFR from luminosity at 1.4 GHz murphy et al., 2011)
% We observed ASKAP~J0055$–$2558 with the X-ray telescope (XRT, \citealp{Burrows:2005}) on board {\it Swift} on August\,8 2024 for 3.6\,ks (ID 00016752001; PI: Gulati). We performed {\it Swift}/XRT data analysis using \textsc{xrtpipeline} and following the standard guidelines (e.g., \citealp{Evans:2009}). No X-ray counterpart was detected in the 0.2--12, 0.2--2, 2--12\,keV images. The 90\% upper limits on the flux in the 0.2--2, 2--12 and 0.2--12\,keV ranges are $5.8\times10^{-14}$, $2.2\times10^{-14}$ and $3.6\times10^{-14}\rm\,erg\,cm^{-2}\,s^{-1}$, respectively, where count rate is 6.4e-4 ct/s. The fluxes were obtained assuming a power-law emission with a photon index $\Gamma=1.7$ and as the transient is located outside the main galaxy, it's plausible to take simply the line-of-sight Galactic value, which is $2\times10^{20}\:cm^{-2}$ using \texttt{PIMMS}\footnote{\url{https://url.au.m.mimecastprotect.com/s/pONmCOMKzVTvYJJpycEfMsG0qKk?domain=heasarc.gsfc.nasa.gov}}. Assuming a distance of 543\,Mpc for the potential host galaxy (see Section \ref{sec:host_galaxy}) we also calculate the luminosity limits from the X-ray non-detections - 0.2-12 keV: L < 2.3e42 erg/s
% 0.2-2 keV: L < 0.9e42 erg/s
% 2-12 keV:  L < 1.3e42 erg/s.
% ASKAP J0055$–$2558 was identified during a search for radio afterglows associated with archival gravitational wave events using ASKAP \citep{2025MNRAS.538.2676G}. 
% The transient lies within the 90\% localization region of GW190814 \citep[a candidate neutron star–black hole merger;][]{2021PhRvX..11b1053A} and was identified during follow-up analysis of archival survey data \citep[see Section~\ref{s_surveys};][]{2020PASA...37...48M, 2020PASP..132c5001L, 2021PASA...38...54M, 2022MNRAS.510.3794D}.
% The source was undetected in both the RACS and the Very Large Array Sky Survey \citep[VLASS;][]{2020PASP..132c5001L} prior to 2022, but subsequently brightened by a factor of ~20 in under 250 days and has been steadily declining in flux for over 1000 days. 
% Based on the typical localisations we estimate a chance coincidence of Z 
% For short time windows ($\lesssim 10$~yr), the per-burst chance coincidence probability is only a few percent, but for the full $\sim 30$-year span it exceeds 50\%. Given the large localization regions of many GRBs and the high all-sky burst rate, these spatial matches are fully consistent with random alignment, and we therefore do not consider any of them to be a strong counterpart.
% \red{Artem will put in some calculations showing an ESE is not possible. -- Have put it in now. In my view there's not much point moving this little into a separate appendix but the second paragraph could be omitted in principle (in which case $\kappa/\gamma$  would need to be culled from the following paragraph.}
%While boosting the flux density by a factor of 20 is certainly possible, doing so across a broad band would require implausible fine-tuning, effectively ruling out an extreme scattering event interpretation as well (see Appendix~\ref{app:mw}).
% It is very unlikely that the significant, over a factor of 20, brightening observed in $\rm \source$ is due to an extreme scattering event (ESE). While there is essentially no limit on the magnification $\mu$ due to lensing by a large-scale plasma lens \citep[\textit{e.g.},][]{2016ApJ...817..176T}, the fractional bandwidth of simultaneous high magnification is expected to be low, of order $\Delta\nu/\nu\propto1/\mu$, unless a highly contrived plasma density profile is invoked.

% Specifically, one can write for the magnification of an image as a function of frequency:
% \begin{equation}
%     \mu(\nu)=\left|1-2\frac{\nu_0^2}{\nu^2}\kappa+\frac{\nu_0^4}{\nu^4}(\kappa^2-\gamma^2)\right|^{-1}
% \end{equation}
% with $\kappa$ and $\gamma$ combinations of the second derivatives of the plasma column, and maintaining high magnification over a broad range of $\nu$ requires the last two terms on the right-hand side to keep a value very near 1 over that range. While $\kappa, \gamma$ themselves depend on frequency via the chromaticity in the position of the image, the latter is determined from an equation involving first derivatives of the column. Thus, although it is in principle possible to fit an arbitrary (sufficiently smooth) dynamic spectrum with a 2D plasma lens, it would require a highly unnatural plasma arrangement.

% It is significantly easier to achieve broadband \emph{de}-magnification using a highly overfocused lens -- \textit{i.e.}, where $|\kappa|$ and/or $\gamma$ are well in excess of unity at the centre of the required band. This would imply interpreting non-detections in early epochs as due to de-magnification and subsequent brightening as return to its intrinsic brightness, possibly undergoing a modest enhancement in the trailing 'horn' of the classic ESE light curve \citep{1987Natur.326..675F}. The light curves shown in Figure~\ref{fig:lightcurve} are consistent with the higher-to-lower frequencies direction of the caustic sweep expected in the trailing half of the ESE \citep{2016Sci...351..354B} and lack of constraints on the\source brightness prior to 2019 or its intrinsic spectrum does not allow to rule out this scenario completely. However, the continuing decline of 9 GHz and 5.5 GHz light curves years after their presumed peak with little variation of flux below 2 GHz makes this interpretation increasingly unlikely.
% The observed luminosity, duration, and multi-wavelength behavior of ASKAP J0055-–2558 make it a compelling candidate for a jetted TDE involving an intermediate-mass black hole (IMBH), or the orphan afterglow of a l-GRB observed off-axis -- both farely undetected, long-lived, luminous transients \citep{2018NatAs...2..656L,2022ApJ...924...16M}.
% \red{To further distinguish the nature of the transient's origin between an H II region and AGN, we analyzed optical spectra at its location and compared it to the Baldwin, Phillips and Terlevich (BPT) diagram \citep{1981PASP...93....5B}. The key BPT line ratios (see Table~\ref{Table:Galaxy_params}) place the emission within the H\,\textsc{ii} region regime of the BPT diagram, indicating photoionization by young, massive stars and disfavoring an AGN origin.}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/GW190814_interesting_source_closure_relation_fit.pdf}
   
%     \caption{Decay time versus observation date. Horizontal dashed lines show the temporal decay index derived from the 9 GHz light curve (Section \ref{ss_spectra_temp_modelling}), assuming explosion dates shifted by 1 (blue), 500 (teal), and 1000 (green) days prior to the first radio detection, reflecting uncertainty in the outflow launch time. The expected decay rates are computed by propagating the spectral index (also from Section \ref{ss_spectra_temp_modelling}) through the Newtonian closure relations of \citet{2013NewAR..57..141G}, for both homogeneous ISM (black points) and wind-like (red points) environments.}
%     \label{Figure:closure_relation}
% \end{figure}


% Applying the formalism of a homogeneous and inhomogenous external FFA model from \citet{2022MNRAS.512.5358R}, we find that for a spectral turnover near 1~GHz, the optically thick portion of the spectrum would be characterized by an exponentially steep decline toward lower frequencies significantly sharper than the $S_\nu \propto \nu^{2.5}$ rise expected from SSA for homogenous model but would be plausible for an inhomogenous model. Lack of Multiwavelength Counterparts (Caveat) is the most challenging aspect for a direct fit. While some GPS/CSS sources are associated with optical and X-ray emission from their host galaxies or AGN, the extreme faintness you observe (optical <28 mag, IR <24 mag, X-ray. In summary, the radio spectral and temporal characteristics of your transient strongly point towards a GPS source. The absence of multiwavelength counterparts would be a significant observational constraint that would need to be addressed, potentially suggesting an obscured or unique type of GPS source. Given that there is a star forming galaxy nearby with an extremely low chance coincidence, it is much more likely to be associated with that.
% Instead, the result is consistent with the $t^{-0.6}$ evolution predicted for the ordering $\nu_a < \nu_m < \nu_c$ \citep{2021ApJ...907...60M}, suggesting that $\nu_a$ and $\nu_m$ are nearly coincident in frequency . 

  

% This gradual evolution in the sub-relativistic phase provides a natural explanation for the near-constancy of $\nu_a$ observed in ASKAP~J0055$-$2558 over extended timescales.

% The 0.9\,GHz flux density is initially low, which is consistent with the source being optically thick at 0.9\,GHz. Between 250 and 1000 days after the first radio detection, the average 0.9\,GHz flux declines by a factor of , with substantial scatter. 
% As the source expands over time, the modulation from scintillation is expected to diminish, particularly at lower frequencies. 
% However, the variability observed at earlier epochs complicates efforts to isolate this trend, and as a result, the long-term decline at 0.9\,GHz remains poorly constrained.
% For an off-axis jet, \citet{2023MNRAS.524.1386B} also show that the further our line of sight is from the jet core the more underestimated our physical parameters, hence, the values calculated in Section~\ref{ss_eqipartition_analysis} should be taken as a lower limit in the case of an off-axis jet. 
% This spectral behavior and longevity make it a strong analog to ASKAP~J0055$–$2558. 
% and a compelling candidate for an orphan afterglow or off-nuclear jetted TDE.



% \subsection{Cygnus A-2}

% Cygnus A-2 was discovered by \citet{2017ApJ...841..117P} during a reanalysis of archival VLA data. The source exhibits a peaked spectrum around $\sim$15\,GHz, with an optically thin spectral index of $\alpha_{\mathrm{thin}} = -0.6 \pm 0.1$, consistent with synchrotron emission. Its flux increased by at least a factor of four over the 26 years since its last non-detection and appears to fade extremely slowly over the two years of observations (see Figure \ref{Figure:CygnusA-2}). Because Cygnus A is an extremely bright radio galaxy ($\sim$1000s of mJy), disentangling the transient emission with wide-field arcsecond resolution surveys like RACS or VLASS is not feasible.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/CygusA-2.pdf}
%     \caption{Radio light curve of Cygnus A-2, incorporating data from \citet{2017ApJ...841..117P}. Different colors represent different observing frequencies, and downward arrows indicate 5$\sigma$ upper limits.}
%     \label{Figure:CygnusA-2}
% \end{figure}
% \subsubsection{Star-forming Galaxies}

% In the case where the galaxy is undergoing a recent or ongoing starburst, the mass-to-light ratio is expected to be significantly lower, due to the dominance of young, massive stars. For blue, actively star-forming galaxies, typical $R$-band mass-to-light ratios are in the range $(M/L)_r \approx 0.5$--$1.0$ \cite{Kannappan2004,McGaugh2014}. Assuming $(M/L)_r = 0.8$ as representative of a starburst galaxy, the stellar mass becomes $2 \times 10^9~M_\odot$. This suggests that the stellar mass estimate could be a factor of $\sim 3$--4 lower than that derived using a typical value for quiescent or mixed-population galaxies.


% A similar analysis for the region containing the transient and the far-left galaxy yields $F_{\mathrm{H}\alpha} = 2.783 \times 10^{-16}$\,erg\,s$^{-1}$\,cm$^{-2}$ and $F_{\mathrm{H}\beta} = 6.49 \times 10^{-17}$\,erg\,s$^{-1}$\,cm$^{-2}$, gives a Balmer decrement of 4.28. 

% \subsection{BPT Diagram}


% \subsubsection*{Far-Left Blob Region}

% For the smaller star-forming region:
% \[
% A = 8 \times (0.6789\arcsec)^2 = 8 \times (1.8~\mathrm{kpc})^2 = 25.92~\mathrm{kpc}^2
% \]
% \[
% \Sigma_{\mathrm{SFR}} = \frac{0.078}{25.92} = 3.01 \times 10^{-3}~M_\odot~\mathrm{yr}^{-1}~\mathrm{kpc}^{-2}
% \]
% \[
% \Sigma_{\mathrm{gas}} = \left( \frac{3.01 \times 10^{-3}}{2.5 \times 10^{-4}} \right)^{1/1.4} \approx 5.89~M_\odot~\mathrm{pc}^{-2}
% \]
% \[
% M_{\mathrm{gas}} = 5.89 \times 10^6~M_\odot~\mathrm{kpc}^{-2} \times 25.92~\mathrm{kpc}^2 \approx 1.5 \times 10^8~M_\odot
% \]

% Similarly, the $R$-band apparent magnitude for the galaxy component near our transient is $m_r = 23.97$, corresponding to a stellar mass ofan absolute magnitude of $M_r = -14.7$. Using the same $(M/L)_r = 3$:
% \begin{equation}
% \frac{L_r}{L_{r,\odot}} = 10^{0.4(4.46 - (-14.7))} \approx 10^{7.7}
% \end{equation}
% \begin{equation}
% M_* = 3 \times 10^{7.7} \approx 1.4 \times 10^8~M_\odot
% \end{equation}

% Across all assumed geometries, this profile supports a scenario involving a weak jet-driven explosions, reflecting an uneven distribution of energy across relativistic and slower ejecta unlike in on-axis GRBs \citep{2012ApJ...750...68L, 2013ApJ...778...18M}.

% Results are shown for different assumed outflow geometries: spherical and conical with opening angles of $5^\circ$, $15^\circ$, and $30^\circ$. The number of degrees of freedom are 7.Best-fit power-law slopes ($k$) and reduced chi-squared values ($\chi^2_{\rm red}$) for two relations: (1) energy versus outflow velocity, $E_{\rm eq} \propto (\Gamma\beta)^k$, and (2) ambient electron density versus scaled radius, $n_e \propto (R_{\rm eq}/R_{s})^k$ 


% Physical outflow parameters for ASKAP J0055–2558 derived from equipartition modeling of the radio spectra, assuming different outflow geometries. For each epoch, we list the equipartition radius ($R_{\rm eq}$), energy ($E_{\rm eq}$), outflow velocity ($\beta = v/c$), ejected mass ($M_{\rm ej}$), magnetic field strength ($B$), and ambient number density ($n_0$). Uncertainties represent 1$\sigma$ credible intervals derived from MCMC fitting of the SBPL spectral parameters shown in Figure~\ref{fig:SBPL_params}.

\red{Deep Magellan imaging also reveals an additional flux excess coincident with the transient. In the context of a TDE scenario, this excess could correspond to a globular cluster associated with the host galaxy. If interpreted as an NSC, the inferred absolute magnitude is $M_g\approx-14.71$. Applying typical scaling relation between host galaxy magnitude and central black hole mass from \citep{Tundo2007}:}
% \begin{equation}
%      \log(M_{\rm BH}/M_\odot) = (8.68 \pm 0.1) - \frac{(1.30 \pm 0.15)}{2.5} (M_r + 22) \end{equation}

% \red{which has a scatter of 0.3 dex. Assuming that the relation is the same for $g$-band magnitudes, we would expect an MBH of mass $\log M_{\text{BH}}/M_{\odot}\approx4.9$, if all the emission at the radio transient position is associated with a NSC star cluster hosting an MBH. Incorporating the scatter, we consider $\log M_{\text{BH}}/M_{\odot}\approx5.2$ as a conservative upper limit on the black hole mass, placing the source firmly in the intermediate-mass black hole regime. We caution that the observed flux excess may instead arise from the host’s tidal features, which are not fully captured by the \texttt{Scarlet} model. In this case, the true black hole mass would be lower, and the NSC interpretation less secure. Thus, while an IMBH TDE remains a viable explanation, the evidence should be regarded as suggestive rather than conclusive.}

% The final combined image is shown in Fig.~\ref{fig:combined_overlay_spectra}. 

% \begin{figure}[]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/GW190814_interesting_lightcurve.pdf}
   
%     \caption{Radio light curves of ASKAP J0055–2558. The data span frequencies from 0.4 to 9 GHz, obtained with ASKAP ("$\circ$"), ATCA ("$\diamond$"), GMRT ("$\square$") and VLA ("$\triangle$"). Different frequency bands are represented by distinct colors. Detections are shown as circles; 5$\sigma$ upper limits are indicated by downward arrows.}
%     \label{fig:lightcurve}
% \end{figure}

% \begin{figure}[]
%     \centering
%     \includegraphics[width=0.465\textwidth]{figures/GW190814_interesting_SBPL_fits.pdf}
   
%     \caption{Radio spectral evolution of \source\ over nine ATCA epochs from 2023 to 2025, assuming synchrotron emission with the spectral peak corresponding to the self-absorption break. The errors on datapoints include both measurement and ISS errors. Solid dark lines show the best-fit spectra, while lighter lines represent 50 random samples from the MCMC posterior distribution, illustrating the approximate fit uncertainties.}
%     \label{fig:spectral_fits}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/X-ray_opt_extracted_spectra.pdf}
   
    \caption{Near simultaneous optical constraints from ZTF g-band limiting magnitudes ("$\triangledown$"), shown together with 90\% X-ray (0.2–12 keV) upper limits (dashed line). The extracted radio spectra are overplotted for comparison.}
    \label{Figure:opt_xray_lims}
\end{figure}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/ZTF_upper_lims.pdf}
    \caption{ZTF g-,r- and i-band limiting magnitudes for the transient. The date of the last radio non-detection is marked, along with the epoch of the first radio detection}
    \label{fig:ztf_lims}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/Paper_spectra_ASKAPJ0055_transient_position.pdf}
    \caption{Spectra obtained with Keck KCWI and KCRM at the position of the transient, with emission lines fitted using the \texttt{LIME} package.}
    \label{fig:keck_spectra_transient}
\end{figure*}

\begin{table}[h]
\centering
\caption{Probability of chance coincidence from Monte Carlo simulations.}
\begin{tabular}{r r r}
\hline
$Y$ (yr) & GRBs in window & $f_{\mathrm{hit}}$ \\
\hline
1  & 0  & --- \\
5  & 2  & 0.01095\ (\(\approx 1.1\%\)) \\
10 & 3  & 0.02520\ (\(\approx 2.5\%\)) \\
20 & 12 & 0.23765\ (\(\approx 23.8\%\)) \\
30 & 54 & 0.55485\ (\(\approx 55.5\%\)) \\
\hline
\end{tabular}
\end{table}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/ISS_source_size_scattering_disk_size.pdf}
    \caption{Comparison of source size estimates with scattering constraints. The solid lines show the expected refractive interstellar scintillation (RISS) scattering disk size as a function of frequency. The dashed lines (in different colors) represent the preliminary source sizes inferred from equipartition analysis under different assumed geometries. The red dashed line marks the mean source size adopted in this work.}
    \label{fig:ISS_scattering_disk_source_size}
\end{figure*}

\section{Comparison to Similar Radio Transients}
\label{sec:pop}

The search for orphan radio transients has been ongoing since the work of \citet{2002ApJ...576..923L}, but progress has been limited by the difficulty of confirming candidates in the absence of extensive multifrequency coverage, multiwavelength counterparts, and long-term monitoring. In this section, we present two known radio transients that share some properties with ASKAP~J0055$-$2558. While FIRST J141918.9+394036 \citep{2018ApJ...866L..22L,mooley_late-time_2022} is a long-lived, luminous peaked-spectrum event and a direct analog to our source, we do not discuss it further here, as it is already a well-studied and confirmed orphan afterglow candidate that has since faded to non-detections in current VLASS data. For the two transients we do present, we have incorporated more recent ASKAP observations into their light curves, but the available data remain insufficient to establish a firm classification.

\subsection{J060938$-$333508}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/J060938-333508.pdf}
    \caption{Radio light curve of J060938–333508, incorporating data from \citet{bannister_22-yr_2011} along with all available measurements from RACS and VLASS. Different colors represent different observing frequencies, and downward arrows indicate 5$\sigma$ upper limits. The dashed red line separates the previously published data and new observations.}
    \label{Figure:J060938-333508}
\end{figure}

J060938$-$333508 was discovered in transient searches using data from the Molonglo Observatory Synthesis Telescope (MOST) and the NRAO VLA Sky Survey \citep[NVSS;][]{1998AJ....115.1693C}, as reported by \citet{2011MNRAS.418.2813B}. The source brightened by a factor of $\sim$8 over less than a decade, rising from non-detections. J060938$-$333508 remains detectable 15 years after discovery, although its flux has decreased by a factor of five from the initial 21.3\,mJy (see Fig. \ref{Figure:J060938-333508}). It retains a steep spectrum at late times, with a spectral index of $-1.1\pm0.1$ between 0.9–3 GHz RACS and VLASS observations, consistent with synchrotron emission. 

The source lies approximately 7\,kpc from the SBab D-type galaxy Fairall 1138 at $z = 0.037$ \citep[$P_{cc} = 0.75\%$; calculated following the method in ][]{2002AJ....123.1111B}, suggesting a likely physical association. Assuming this association, the inferred peak spectral luminosity at 843\,MHz is $\sim10^{29}\:\mathrm{erg\:s^{-1}\:Hz^{-1}}$, consistent with the radio luminosities of jetted TDEs or long GRBs. 

The transient is located at a projected offset of 460\,pc from the nucleus of the radio-loud galaxy Cygnus A \citep[$P_{cc} < 10^{-4}$][]{2017ApJ...841..117P}, within a complex, gas-rich inner region \citep[][]{1976ApJ...206..883V,2003ApJ...597..823C}. Its inferred radio luminosity is $L_\nu \sim 3 \times 10^{29}\:\mathrm{erg\:s^{-1}\:Hz^{-1}}$, compatible with l-GRBs and jetted TDEs. Furthermore, multi-wavelength constraints, particularly in the X-ray \citep{2019MNRAS.486.3388D}, rule out steady AGN activity, supporting a transient origin. Spectral behavior,  longevity and off-nuclear emission in a star forming environment point to this transient being an analog to ASKAP~J0055$–$2558.


\subsection{ASKAP J175036.1$-$181454}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/J175036.1−181454.pdf}
    \caption{Radio light curve of J175036.1-181454, incorporating data from \citet{2023MNRAS.523.4029L} along with all available measurements from RACS, VAST and VLASS. Different colors represent different observing frequencies, and downward arrows indicate 5$\sigma$ upper limits. The dashed red line separates the previously published data and new observations.}
    \label{Figure:J175036.1−181454}
\end{figure}

ASKAP J175036.1$-$181454 was identified in an ASKAP search for orphan afterglows by \citet{2023MNRAS.523.4029L}. The source rose from non-detections with an initially inverted spectrum, evolving into a peaked profile at 2.3,GHz. At 0.9,GHz the rise remains unconstrained, whereas at 3\,GHz the light curve brightened by a factor of $\sim$3 relative to the non-detection limit before subsequently declining. The optically thin spectral index of $\sim -0.9$ indicates synchrotron emission. The source remains detectable, declining and variable more than 1000 days after discovery in VAST monitoring (see Fig. \ref{Figure:J175036.1−181454} updated with all available radio data). We calculated the modulation index as the standard deviation of the residuals from a log–log fit to the flux density decline with time, obtaining a value of $\sim$7.2\%.

The source lies $\sim$2\,kpc from a host galaxy at $z = 0.25$ with $P_{cc} = 0.6\%$, supporting a likely association. Its radio luminosity at 9\,GHz, measured 226 days after discovery, is $\sim10^{30}\:\mathrm{erg\:s^{-1}\:Hz^{-1}}$,comparable to our transient. Based on the \citet{2002astro.ph..7156C} scattering model, the transition frequency for this line of sight is 68.5\,GHz, and the first Fresnel zone at 0.9\,GHz corresponds to an angular scale of 7910\,µas and a modulation index of 8.5\%. At a redshift of 0.25, this implies that the source size after a 1000 days must remain extremely compact compared to the large scattering disk scale of $\rm \sim0.7\,Mpc$. Overall, the long-lived, luminous, and peaked synchrotron evolution of ASKAP J175036.1$-$181454 makes it a strong analog to our transient and a compelling candidate for an orphan afterglow, as also noted by \citet{2023MNRAS.523.4029L}, or a tidal disruption event on an IMBH.

To reliably detect and confirm \source\-like events in the future, comprehensive multi-frequency coverage, systematic multiwavelength follow-up, and long-term monitoring will be essential. Upcoming surveys such as VAST, with their improved cadence and regular sampling, will help address some of these limitations. Nonetheless, these examples highlight the challenges involved and underscore the importance of careful, sustained follow-up in the search for orphan events.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/beta_eq_N.pdf}
   
    \caption{Equipartition-based Newtonian velocity ($\beta_{\rm eq,N}$) versus epoch of observation. Different colors represent different collimated outflow geometries. Solid lines show $\beta_{\rm eq,N}$ for ASKAP~J0055$–$2558 using the first radio detection date (2022-02-04) as the reference. Since $\beta_{\rm eq,N} \propto t^{-1}$, dashed lines show the evolution assuming an outflow launch 1000 days prior to detection. The gray shaded region marks the on/off-axis threshold; values above 0.23 suggest the outflow may have originated as a relativistic jet that has since decelerated into the Newtonian regime.}
    \label{Figure:beta_eq_N}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/GW190814_interesting_source_radio_postage_stamps.pdf}
   
    \caption{Radio postage stamps of ASKAP J0055–2558 at 944\,MHz (ASKAP) and 9.0\,GHz (ATCA). Left–to–right: the last ASKAP non-detection (AS111) on 2021-05-29 prior to the source’s emergence; the first ASKAP/RACS detection on 2022-04-15; the first ATCA follow-up on 2023-05-04; and the most recent ATCA observation on 2025-03-20.}
    \label{fig:postage_stamps}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/SBPL_joint_ISS_corner_plot.png}
    \caption{ Corner plot showing the posterior distributions from the joint MCMC fitting of the modified smoothly broken power-law (SBPL) model to all available radio data.}
    \label{fig:SBPL_fits_corner_plot}
\end{figure*}

conducted with \texttt{MIRIAD} tasks \mbox{} \texttt{uvflag} and \texttt{pgflag}, respectively
\texttt{INVERT}, \texttt{CLEAN} and \texttt{RESTOR} to obtain the final images. For each observation, we measure the flux density of a detected source by 
fitting a point-source model to the restored image using the {\sc Miriad} task {\sc imfit} and report a non-detection using the rms sensitivity obtained from the residual image. 
The $1\sigma$ errors reported are purely statistical, as the systematic errors are expected to be much smaller \citep[$\lesssim 5$ per cent; e.g.,][]{Reynolds1994,Tingay2003}.

% \subsection{Galaxy Stellar Mass}

% The $R$-band apparent magnitude of the main galaxy is $m_r = 19.58$. The absolute magnitude is then calculated as:
% \begin{equation}
% M_r = m_r - 5\log_{10}(d) + 5 = 19.58 - 5\log_{10}(543 \text{Mpc}) + 5 = -19
% \end{equation}

% The absolute magnitude of the Sun in the $r$-band is $M_{r,\odot} = 4.46$. The ratio of luminosities is given by:
% \begin{equation}
% \frac{L_r}{L_{r,\odot}} = 10^{0.4(M_{r,\odot} - M_r)} = 10^{0.4(4.46 - (-19))} \approx 10^{9.4}
% \end{equation}

% We can estimate the stellar mass using a mass-to-light ratio $(M/L)_r$. Empirical calibrations \citep[e.g.,][]{2003ApJS..149..289B} provide $(M/L)_r$ as a function of galaxy color. Assuming $(M/L)_r = 3$, the stellar mass of the galaxy is:
% \begin{equation}
% M_* = \left( \frac{M}{L} \right)_r \times \frac{L_r}{L_{r,\odot}} = 3 \times 10^{9.4} \approx 7.5 \times 10^9~M_\odot
% \end{equation}






% \subsection{Star Formation Rate from UV imaging}

% To estimate the star formation rate (SFR) from the ultraviolet (UV) emission of the galaxy, we use the observed far-UV (FUV) flux density corrected for dust attenuation using extinction laws for both star-forming and Milky Way-like galaxies . The intrinsic UV luminosity is related to the observed flux via $L_\nu = 4\pi D_L^2$, where $D_L$ is the luminosity distance in cm, and $F_\nu$ is the FUV flux density in $erg\:s^{-1}cm^{-2}Hz^{-1}$. The observed FUV luminosity is then corrected for internal extinction using the UV color FUV - NUV. 


% \subsubsection{Star-Forming Galaxies}

% For star-forming galaxies, the Calzetti extinction law \citep{2000ApJ...533..682C,2007ApJS..173..267S} gives the attenuation in the FUV as:

% \begin{equation}
% A_\mathrm{FUV} = 3.32 \times (\mathrm{FUV} - \mathrm{NUV}) + 0.22
% \end{equation}

% The corresponding corrected luminosity is:

% \begin{equation}
% L_{\nu,\text{corr}} = L_\nu \times 10^{0.4 A_\mathrm{FUV}}
% \label{kenn-schmidt}
% \end{equation}

% and the star formation rate is calculated using the \citep{2011ApJ...741..124H} relation (assuming a Salpeter IMF):

% \begin{equation}
% \mathrm{SFR}~[M_\odot~\text{yr}^{-1}] = 1.4 \times 10^{-28} \times L_{\nu,\text{corr}}~[\text{erg s}^{-1} \text{Hz}^{-1}]
% \end{equation}

% Given a $F_{FUV} = 8.86e^{-6}$\,Jy and FUV and NUV magnitudes of 21.532 and 21.064, we get an extinction of 1.7 mag and a corresponding SFR of 2.24 $M_\odot~\text{yr}^{-1}$.

% \subsubsection{Milky way-like Galaxies}

% For a Milky Way-like extinction curve based on the Cardelli law \citep{1989ApJ...345..245C,2011ApJ...741..124H}, the FUV attenuation can be approximated as:

% \begin{equation}
% A_\mathrm{FUV} = 8.24 \times (\mathrm{FUV} - \mathrm{NUV}) - 0.67
% \end{equation}

% with the SFR estimated using the  equation \ref{kenn-schmidt}. These two methods provide a range of plausible SFR values depending on the assumed dust extinction law. The corresponding SFR is 8.23 $M_\odot~\text{yr}^{-1}$.



% \subsection{Galaxy Gas Mass}

% We estimate the total gas mass of the host galaxy and its star-forming regions using the Kennicutt-Schmidt relation \citep{1998ApJ...498..541K}, which relates the gas surface density to the surface density of star formation via a power-law:

% \begin{equation}
% \Sigma_{\mathrm{gas}} = \left( \frac{\Sigma_{\mathrm{SFR}}}{2.5 \times 10^{-4}} \right)^{1/1.4} \quad M_\odot~\mathrm{pc}^{-2}
% \end{equation}

% The projected area of the main galaxy, as estimated from imaging, is $84.24~\mathrm{kpc}^2$. Using a total star formation rate of $2.24~M_\odot~\mathrm{yr}^{-1}$ derived under the Calzetti extinction law, the corresponding surface density of star formation is:

% \[
% \Sigma_{\mathrm{SFR}} = \frac{2.24}{84.24} = 0.027~M_\odot~\mathrm{yr}^{-1}~\mathrm{kpc}^{-2}
% \]

% For comparison, the value obtained under the Cardelli extinction law is $\Sigma_{\mathrm{SFR}} = 0.098~M_\odot~\mathrm{yr}^{-1}~\mathrm{kpc}^{-2}$. Applying the Kennicutt-Schmidt relation yields gas surface densities of:

% \[
% \Sigma_{\mathrm{gas}} = 28.3~M_\odot~\mathrm{pc}^{-2} \quad \text{(Calzetti)}, \quad \Sigma_{\mathrm{gas}} = 71.2~M_\odot~\mathrm{pc}^{-2} \quad \text{(Cardelli)}
% \]

% The total gas mass is then calculated as:

% \[
% M_{\mathrm{gas}} = \Sigma_{\mathrm{gas}} \times A
% \]

% resulting in total gas masses of:

% \[
% M_{\mathrm{gas}} = 2.39 \times 10^9~M_\odot \quad \text{(Calzetti)}, \quad M_{\mathrm{gas}} = 6.00 \times 10^9~M_\odot \quad \text{(Cardelli)}
% \]



% \subsection{Dust Extinction and Flux Correction}

% The intrinsic (dust-free) ratio of the Balmer decrement, i.e., the flux ratio of H$\alpha$ (6563\,\AA) to H$\beta$ (4861\,\AA), is theoretically expected to be $2.86$ for typical nebular conditions \citep{1989agna.book.....O}. For the main galaxy, we measure an observed H$\alpha$ flux of $F_{\mathrm{H}\alpha} = 5.95 \times 10^{-16}$\,erg\,s$^{-1}$\,cm$^{-2}$ and H$\beta$ flux of $F_{\mathrm{H}\beta} = 1.49 \times 10^{-16}$\,erg\,s$^{-1}$\,cm$^{-2}$. The observed Balmer decrement is therefore:

% \begin{equation}
% \frac{F_{\mathrm{H}\alpha}}{F_{\mathrm{H}\beta}} = \frac{5.95 \times 10^{-16}}{1.49 \times 10^{-16}} \approx 3.99
% \end{equation}



% The color excess $E(B-V)$ can be derived using:

% \begin{equation}
% E(B-V) = \frac{2.5}{k(\mathrm{H}\beta) - k(\mathrm{H}\alpha)} \log_{10} \left( \frac{(F_{\mathrm{H}\alpha}/F_{\mathrm{H}\beta})_{\text{obs}}}{2.86} \right)
% \end{equation}

% Here, $k(\lambda)$ is the extinction curve at the given wavelength. For star-forming galaxies we use $R_V = 4.05$, where $k(\mathrm{H}\alpha) = 3.325$, $k(\mathrm{H}\beta) = 4.598$, giving an E(B-V) of 0.27 \citep{2000ApJ...533..682C}. For Milky-way like galaxies, we use $R_V = 3.1$, where $k(\mathrm{H}\alpha) = 2.535$, $k(\mathrm{H}\beta) = 3.609$, which gives an E(B-V) of 0.37 \citep{1989ApJ...345..245C}. The extinction in $V$-band is then given by $A_V = R_V \times E(B-V)$, yielding $A_V \approx 1.15$ \citep{1989ApJ...345..245C} and $A_V \approx 1.09$ \citep{2000ApJ...533..682C} To correct line fluxes for dust extinction, we use the redenning law \citep{1994ApJ...429..582C,1997AIPC..408..403C}

% \begin{equation}
% F_{\text{corr}} = F_{\text{obs}} \times 10^{0.4 A_\lambda}
% \end{equation}

% where $A_\lambda = k(\lambda) \cdot E(B-V)$. This correction is applied individually at each wavelength of interest using the chosen extinction law.






% \subsection{Ionisation Ratio}

% The [O\,\textsc{iii}] emission lines at 4959\,\AA\ and 5007\,\AA\ are both produced by doubly ionized oxygen (O$^{2+}$), with the flux ratio between them fixed by atomic transition probabilities. Theoretical predictions give $\frac{F_{5007}}{F_{4959}} \approx 2.98$ \citep{2007MNRAS.374.1181D} . To estimate the total [O\,\textsc{iii}] emission when only the 4959\,\AA\ line is available, we approximate:

% \begin{equation}
% F_{[\mathrm{O\,III}]} \approx F_{4959} + F_{5007} \approx (1 + 2.98) \times F_{4959} \approx 4 \times F_{4959}
% \end{equation}

% The [O\,\textsc{iii}]/[O\,\textsc{ii}] line ratio serves as a widely used diagnostic of the ionization state of gas in galaxies. [O\,\textsc{ii}] $\lambda$3727 traces singly ionized oxygen (O$^{+}$), associated with lower-energy photons, while [O\,\textsc{iii}] emission arises from higher ionization zones powered by young, massive stars or AGN activity.
% The corrected [O\,\textsc{iii}] flux for the main galaxy using calzetti correction is $2.05 \times 10^{-15}~\mathrm{erg~s^{-1}~cm^{-2}}$ and the [O\,\textsc{ii}] flux is $2.32 \times 10^{-15}~\mathrm{erg~s^{-1}~cm^{-2}}$, giving an ionisation ratio of 0.88. The corrected [O\,\textsc{iii}] flux for the main galaxy using calzetti correction is $2.25 \times 10^{-15}~\mathrm{erg~s^{-1}~cm^{-2}}$ and the [O\,\textsc{ii}] flux is $2.45 \times 10^{-15}~\mathrm{erg~s^{-1}~cm^{-2}}$, giving an ionisation ratio of 0.92. 

To assess whether any of the spatially coincident GRBs are likely to be genuine counterparts, we estimated the probability of a chance alignment using a Monte Carlo approach. We fixed the reference date to the epoch of the first radio detection of the source (2022~February~4~UTC) and selected all GRBs within time windows of $Y$ years preceding this date. For each window, we generated $N = 300 \times Y$ simulated GRBs, uniformly distributed over the celestial sphere to match the observed GRB rate of $\sim 300~\mathrm{yr}^{-1}$. We then counted how many of these simulated bursts fell within the localization regions of the actual GRBs in that window.

This procedure was repeated 500 times for each window to account for statistical fluctuations. For each window we computed the mean hit fraction, $f_{\mathrm{hit}}$, defined as the fraction of simulated bursts falling within the actual GRB localizations also interpreted as the probability of chance coincidence. Our Monte Carlo simulations indicate that the probability of a chance coincidence rises steeply with the time window. For a one-year window (\(Y=1\) yr), no GRBs fall within the window and \(f_{\mathrm{hit}}\) is not defined. For \(Y=5\) yr (2 GRBs in the window) we obtain \(f_{\mathrm{hit}}=0.01095\) (\(\approx 1.1\%\)); for \(Y=10\) yr (3 GRBs) \(f_{\mathrm{hit}}=0.02520\) (\(\approx 2.5\%\)); for \(Y=20\) yr (12 GRBs) \(f_{\mathrm{hit}}=0.23765\) (\(\approx 23.8\%\)); and for \(Y=30\) yr (54 GRBs) \(f_{\mathrm{hit}}=0.55485\) (\(\approx 55.5\%\)). Thus, while the chance-coincidence probability is low for \(\lesssim 10\) yr windows, it becomes substantial (\(>50\%\)) over \(\sim 30\) yr.


%% Beginning of file 'sample631.tex'

%%
%% Modified 2022 May  
%%
%% This is a sample manuscript marked up using the
%% AASTeX v6.31 LaTeX 2e macros.
%%
%% AASTeX is now based on Alexey Vikhlinin's emulateapj.cls 
%% (Copyright 2000-2015).  See the classfile for details.

%% AASTeX requires revtex4-1.cls and other external packages such as
%% latexsym, graphicx, amssymb, longtable, and epsf.  Note that as of 
%% Oct 2020, APS now uses revtex4.2e for its journals but remember that 
%% AASTeX v6+ still uses v4.1. All of these external packages should 
%% already be present in the modern TeX distributions but not always.
%% For example, revtex4.1 seems to be missing in the linux version of
%% TexLive 2020. One should be able to get all packages from www.ctan.org.
%% In particular, revtex v4.1 can be found at 
%% https://www.ctan.org/pkg/revtex4-1.

%% The first piece of markup in an AASTeX v6.x document is the \documentclass
%% command. LaTeX will ignore any data that comes before this command. The 
%% documentclass can take an optional argument to modify the output style.
%% The command below calls the preprint style which will produce a tightly 
%% typeset, one-column, single-spaced document.  It is the default and thus
%% does not need to be explicitly stated.
%%
%% using aastex version 6.3
% \documentclass[linenumbers]{aastex631}

%% The default is a single spaced, 10 point font, single spaced article.
%% There are 5 other style options available via an optional argument. They
%% can be invoked like this:
%%

%% 
%% where the layout options are:
%%
%%  twocolumn   : two text columns, 10 point font, single spaced article.
%%                This is the most compact and represent the final published
%%                derived PDF copy of the accepted manuscript from the publisher
%%  manuscript  : one text column, 12 point font, double spaced article.
%%  preprint    : one text column, 12 point font, single spaced article.  
%%  preprint2   : two text columns, 12 point font, single spaced article.
%%  modern      : a stylish, single text column, 12 point font, article with
%% 		  wider left and right margins. This uses the Daniel
%% 		  Foreman-Mackey and David Hogg design.
%%  RNAAS       : Supresses an abstract. Originally for RNAAS manuscripts 
%%                but now that abstracts are required this is obsolete for
%%                AAS Journals. Authors might need it for other reasons. DO NOT
%%                use \begin{abstract} and \end{abstract} with this style.
%%
%% Note that you can submit to the AAS Journals in any of these 6 styles.
%%
%% There are other optional arguments one can invoke to allow other stylistic
%% actions. The available options are:
%%
%%   astrosymb    : Loads Astrosymb font and define \astrocommands. 
%%   tighten      : Makes baselineskip slightly smaller, only works with 
%%                  the twocolumn substyle.
%%   times        : uses times font instead of the default
%%   linenumbers  : turn on lineno package.
%%   trackchanges : required to see the revision mark up and print its output
%%   longauthor   : Do not use the more compressed footnote style (default) for 
%%                  the author/collaboration/affiliations. Instead print all
%%                  affiliation information after each name. Creates a much 
%%                  longer author list but may be desirable for short 
%%                  author papers.
%% twocolappendix : make 2 column appendix.
%%   anonymous    : Do not show the authors, affiliations and acknowledgments 
%%                  for dual anonymous review.
%%
%% these can be used in any combination, e.g.
%%
%% \documentclass[twocolumn,linenumbers,trackchanges]{aastex631}
%%
%% AASTeX v6.* now includes \hyperref support. While we have built in specific
%% defaults into the classfile you can manually override them with the
%% \hypersetup command. For example,
%%
%% \hypersetup{linkcolor=red,citecolor=green,filecolor=cyan,urlcolor=magenta}
%%
%% will change the color of the internal links to red, the links to the
%% bibliography to green, the file links to cyan, and the external links to
%% magenta. Additional information on \hyperref options can be found here:
%% https://www.tug.org/applications/hyperref/manual.html#x1-40003
%%
%% Note that in v6.3 "bookmarks" has been changed to "true" in hyperref
%% to improve the accessibility of the compiled pdf file.
%%
%% If you want to create your own macros, you can do so
%% using \newcommand. Your macros should appear before
%% the \begin{document} command.
%%

%% Reintroduced the \received and \accepted commands from AASTeX v5.2
%\received{March 1, 2021}
%\revised{April 1, 2021}
%\accepted{\today}

%% Command to document which AAS Journal the manuscript was submitted to.
%% Adds "Submitted to " the argument.
%\submitjournal{PSJ}

%% For manuscript that include authors in collaborations, AASTeX v6.31
%% builds on the \collaboration command to allow greater freedom to 
%% keep the traditional author+affiliation information but only show
%% subsets. The \collaboration command now must appear AFTER the group
%% of authors in the collaboration and it takes TWO arguments. The last
%% is still the collaboration identifier. The text given in this
%% argument is what will be shown in the manuscript. The first argument
%% is the number of author above the \collaboration command to show with
%% the collaboration text. If there are authors that are not part of any
%% collaboration the \nocollaboration command is used. This command takes
%% one argument which is also the number of authors above to show. A
%% dashed line is shown to indicate no collaboration. This example manuscript
%% shows how these commands work to display specific set of authors 
%% on the front page.
%%
%% For manuscript without any need to use \collaboration the 
%% \AuthorCollaborationLimit command from v6.2 can still be used to 
%% show a subset of authors.
%
%\AuthorCollaborationLimit=2
%
%% will only show Schwarz & Muench on the front page of the manuscript
%% (assuming the \collaboration and \nocollaboration commands are
%% commented out).
%%
%% Note that all of the author will be shown in the published article.
%% This feature is meant to be used prior to acceptance to make the
%% front end of a long author article more manageable. Please do not use
%% this functionality for manuscripts with less than 20 authors. Conversely,
%% please do use this when the number of authors exceeds 40.
%%
%% Use \allauthors at the manuscript end to show the full author list.
%% This command should only be used with \AuthorCollaborationLimit is used.

%% The following command can be used to set the latex table counters.  It
%% is needed in this document because it uses a mix of latex tabular and
%% AASTeX deluxetables.  In general it should not be needed.
%\setcounter{table}{1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% The following section outlines numerous optional output that
%% can be displayed in the front matter or as running meta-data.
%%
%% If you wish, you may supply running head information, although
%% this information may be modified by the editorial offices.
%\shorttitle{AASTeX v6.3.1 Sample article}
%\shortauthors{Schwarz et al.}
%%
%% You can add a light gray and diagonal water-mark to the first page 
%% with this command:
%% \watermark{text}
%% where "text", e.g. DRAFT, is the text to appear.  If the text is 
%% long you can control the water-mark size with:
%% \setwatermarkfontsize{dimension}
%% where dimension is any recognized LaTeX dimension, e.g. pt, in, etc.
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\graphicspath{{./}{figures/}}
%% This is the end of the preamble.  Indicate the beginning of the
%% manuscript itself with \begin{document}.

% \title{Template \aastex Article with Examples: 
% v6.3.1\footnote{Released on March, 1st, 2021}}

%% LaTeX will automatically break titles if they run longer than
%% one line. However, you may use \\ to force a line break if
%% you desire. In v6.31 you can include a footnote in the title.

%% A significant change from earlier AASTEX versions is in the structure for 
%% calling author and affiliations. The change was necessary to implement 
%% auto-indexing of affiliations which prior was a manual process that could 
%% easily be tedious in large author manuscripts.
%%
%% The \author command is the same as before except it now takes an optional
%% argument which is the 16 digit ORCID. The syntax is:
%% \author[xxxx-xxxx-xxxx-xxxx]{Author Name}
%%
%% This will hyperlink the author name to the author's ORCID page. Note that
%% during compilation, LaTeX will do some limited checking of the format of
%% the ID to make sure it is valid. If the "orcid-ID.png" image file is 
%% present or in the LaTeX pathway, the OrcID icon will appear next to
%% the authors name.
%%
%% Use \affiliation for affiliation information. The old \affil is now aliased
%% to \affiliation. AASTeX v6.31 will automatically index these in the header.
%% When a duplicate is found its index will be the same as its previous entry.
%%
%% Note that \altaffilmark and \altaffiltext have been removed and thus 
%% can not be used to document secondary affiliations. If they are used latex
%% will issue a specific error message and quit. Please use multiple 
%% \affiliation calls for to document more than one affiliation.
%%
%% The new \altaffiliation can be used to indicate some secondary information
%% such as fellowships. This command produces a non-numeric footnote that is
%% set away from the numeric \affiliation footnotes.  NOTE that if an
%% \altaffiliation command is used it must come BEFORE the \affiliation call,
%% right after the \author command, in order to place the footnotes in
%% the proper location.
%%
%% Use \email to set provide email addresses. Each \email will appear on its
%% own line so you can put multiple email address in one \email call. A new
%% \correspondingauthor command is available in V6.31 to identify the
%% corresponding author of the manuscript. It is the author's responsibility
%% to make sure this name is also in the author list.
%%
%% While authors can be grouped inside the same \author and \affiliation
%% commands it is better to have a single author for each. This allows for
%% one to exploit all the new benefits and should make book-keeping easier.
%%
%% If done correctly the peer review system will be able to
%% automatically put the author and affiliation information from the manuscript
%% and save the corresponding author the trouble of entering it by hand.

% \author{F.X Timmes}
% \affiliation{Arizona State University}
% \affiliation{AAS Journals Associate Editor-in-Chief}

% \author{Amy Hendrickson}
% \altaffiliation{AASTeX v6+ programmer}
% \affiliation{TeXnology Inc.}

% \author{Julie Steffen}
% \affiliation{AAS Director of Publishing}
% \affiliation{American Astronomical Society \\
% 1667 K Street NW, Suite 800 \\
% Washington, DC 20006, USA}

%% Note that the \and command from previous versions of AASTeX is now
%% depreciated in this version as it is no longer necessary. AASTeX 
%% automatically takes care of all commas and "and"s between authors names.

%% AASTeX 6.31 has the new \collaboration and \nocollaboration commands to
%% provide the collaboration status of a group of authors. These commands 
%% can be used either before or after the list of corresponding authors. The
%% argument for \collaboration is the collaboration identifier. Authors are
%% encouraged to surround collaboration identifiers with ()s. The 
%% \nocollaboration command takes no argument and exists to indicate that
%% the nearby authors are not part of surrounding collaborations.

%% Mark off the abstract in the ``abstract'' environment. 

%% Keywords should appear after the \end{abstract} command. 
%% The AAS Journals now uses Unified Astronomy Thesaurus concepts:
%% https://astrothesaurus.org
%% You will be asked to selected these concepts during the submission process
%% but this old "keyword" functionality is maintained in case authors want
%% to include these concepts in their preprints.
%% From the front matter, we move on to the body of the paper.
%% Sections are demarcated by \section and \subsection, respectively.
%% Observe the use of the LaTeX \label
%% command after the \subsection to give a symbolic KEY to the
%% subsection for cross-referencing in a \ref command.
%% You can use LaTeX's \ref and \label commands to keep track of
%% cross-references to sections, equations, tables, and figures.
%% That way, if you change the order of any elements, LaTeX will
%% automatically renumber them.
%%
%% We recommend that authors also use the natbib \citep
%% and \citet commands to identify citations.  The citations are
%% tied to the reference list via symbolic KEYs. The KEY corresponds
%% to the KEY in the \bibitem in the reference list below. 


%% This command is needed to show the entire author+affiliation list when
%% the collaboration and author truncation commands are used.  It has to
%% go at the end of the manuscript.
%\allauthors

%% Include this line if you are using the \added, \replaced, \deleted
%% commands to see a summary list of all changes at the end of the article.
%\listofchanges

We used \texttt{EzGal} \footnote{\url{https://github.com/cmancone/easyGalaxy}} with a single-burst simple stellar population\footnote{Simple stellar population is an idealized population formed in a single, instantaneous burst with one metallicity. Its spectrum/M/L then evolves only with age.}  \citep{2003MNRAS.344.1000B}, Chabrier initial mass function \citep{2003PASP..115..763C}, solar metallicity and the Sloan $g$ filter (\texttt{sloan\_g}) via \texttt{get\_rest\_ml\_ratios} to get mass to light ratios at ages $0.01$, $1$, and $10$ Gyr. The returned $(M/L)_g=\{0.036,\,0.454,\,4.004\}$. We then get the corresponding stellar masses $M_\star=(M/L)_g\,L_g=\{3.061\times10^{6},\,3.846\times10^{7},\,3.392\times10^{8}\}\,M_\odot$ for the young, intermediate, and old cases, respectively. , where rest–frame $g$-band luminosity is $L_g \simeq 8.47\times10^{7}\,L_{g,\odot}$\footnote{$
\frac{L_g}{L_{g,\odot}} = 10^{-0.4\,(M_g-M_{g,\odot})}$, where $M_{g,\odot}=5.12~\mathrm{(AB)}$}.

 At the low end of this range (young; $M_\star\!\sim\!3\times10^{6}\,M_\odot$), the system would resemble a ``super star cluster'' like those in starburst galaxies (e.g., M82; \citep{2007ApJ...663..844M,2010ARA&A..48..431P}). At the high end (old; $M_\star\!\sim\!10^{8}\,M_\odot$), it approaches the most massive ultra-compact dwarfs (UCDs; \citep{2007A&A...463..119H,2011MNRAS.412.1627C,2008A&A...487..921M,2015ApJ...812L...2L}), and the overall mass range largely overlaps that of nuclear star clusters \citep{2005ApJ...618..237W}. For context, the very massive Virgo UCD M59-UCD3 has a luminosity comparable to our candidate \citep{2015ApJ...812L...2L} and may host a central black hole of mass $\sim\mathrm{few}\times10^{6}\,M_\odot$ \citep{2018ApJ...858..102A}; the similarly extreme M60-UCD1 is also thought to contain a central black hole \citep{2014Natur.513..398S}.

 Similarly, to infer a central black-hole mass,  we apply the cluster relation (Eq.~6 of \citet{2020MNRAS.492.3263G}),
\begin{equation}
\log_{10}\!\left(\frac{M_{\rm bh}}{M_\odot}\right)
=8.22+\frac{\log_{10}(M_{\rm nc}/M_\odot)-7.83}{0.38},
\end{equation}
to the young and intermediate-age masses, obtaining $M_{\rm bh}\approx4.8\times10^{4}\,M_\odot$ (10 Myr) and $M_{\rm bh}\approx3.8\times10^{7}\,M_\odot$ (1 Gyr). We caution that BH–cluster scaling relations can break down at high $M_{\rm nc}$: for the old-mass case ($M_{\rm nc}\sim3.4\times10^{8}\,M_\odot$), the same relation would imply $M_{\rm bh}\sim1.2\times10^{10}\,M_\odot$, exceeding the cluster mass by a factor of $\sim$30; we therefore regard the relation as inapplicable in this regime and do not quote a value. Independently, the extreme luminosity and stellar mass disfavors a classical globular cluster and supports a nuclear star cluster interpretation, supporting the argument for an intermediate mass black-hole. The positional coincidence of this transient with a compact, highly luminous nuclear star cluster, an environment expected to harbor $10^{4}$–$10^{7}\,M_\odot$ black holes also provides support for a TDE on an off-nuclear intermediate-mass black hole.

We conducted our observations with the Meer(more) Karoo Array Telescope (MeerKAT) \citep{Jonas} in L-band (856–1712~MHz) with a usable bandwidth of $\sim770$~MHz in the c856M4k configuration where the correlations were integrated for 8-seconds before saving to disk. Full polarization data for the on-source beam were recorded to disk, but not searched in realtime, using the Pulsar Timing User Supplied Equipment (PTUSE) backend of the MeerKAT pulsar timing project MeerTime described in \cite{meertime2020}. These data were recorded in the PTUSE search mode with a sampling time of $38.28~\mu$s in the \texttt{psrfits} format.

We used pulsar\_miner\footnote{\url{https://github.com/alex88ridolfi/PULSAR_MINER}} \citep[an automated pulsar searching pipeline based on prest][]{2021MNRAS.504.1407R} to do a periodicity search. To run the search more efficiently, we divided the observation into 5~min chunks. We searched for candidates with a dispersion measure (DM) range of up to 50\,pc\,cm$^{-3}$ (double the plausible Galactic DMs along line-of-sight based on the YMW16 model) and periods ranging from 1ms to 10s. We performed acceleration searches in the Fourier domain using the accelsearch routine, with a maximum allowed Doppler-induced Fourier bin drift $z_{max}$ = $\pm$200. We see no convincing pulsar-like candidates in our search with a threshold of 8.

We monitored \source\ for potential short-duration bursts using the Ultra-Wideband Low (UWL) receiver system on Murriyang, the 64 m Parkes radio telescope, which covers a continuous frequency range of 704–4032 MHz \citep{Hobbs2019ultrawide}. We observed it for a total of 1 hour on November 18, 2023. Observations were conducted in single-polarization pulsar search mode, with a spectral resolution of 250 kHz (13312 channels across the full band) and a sampling time of 64 $\mu$s. Data were recorded in the 2-bit PSRFITS search mode format \citep{Hotan04}.

We carried out a search for short-duration bursts using a subbanded search pipeline that integrates single-pulse processing packages such as \textsc{HEIMDALL} \citep{Barsdell12} and \textsc{FETCH} \citep{Aggarwal20}; the pipeline is described in detail by \citet{2022MNRAS.512.3400K}. The search was carried out over a DM range of 0--1000 pc cm$^{-3}$ with a step size of 0.1~pc cm$^{-3}$, using boxcar widths up to 2 minutes. The full band was divided into overlapping subbands of 64, 128, 256, 512, 832, 1664, and 3328 MHz to ensure that no pulses were missed at the band edges. Each candidate identified by \textsc{FETCH} was visually inspected. We found no burst candidates with signal-to-noise ratios greater than 7 in this search. 

 Adopting a distance of 543\,Mpc for the potential host galaxy (Section~\ref{sec:host_galaxy}), the corresponding luminosity upper limits are
$L_{0.2-12}<2.3\times10^{42}\,\mathrm{erg\,s^{-1}}$,
$L_{0.2-2}<9.0\times10^{41}\,\mathrm{erg\,s^{-1}}$, and
$L_{2-12}<1.3\times10^{42}\,\mathrm{erg\,s^{-1}}$. 

% It must be noted that even the most X-ray--luminous supernovae (i.e., the upper end of the Type~IIn population) rarely exceed \(\sim10^{42}\,\mathrm{erg\,s^{-1}}\); accordingly, a supernova counterpart would not be expected to be detectable in our \textit{Swift}/XRT data \citep{2023ApJ...947...42B}.

GRBs are typically followed by a long-lived, multi-wavelength emission known as the afterglow, which follows the brief and high energy prompt phase. As the relativistic blast wave from the GRB, decelerates in the surrounding medium, the Lorentz factor ($\Gamma$) decreases, causing the beaming angle to widen as $\Omega(t) \propto 1/\Gamma(t)^2$ \citep{1997ApJ...482L..29M}. In some instances, even in the absence of a detected prompt GRB, the afterglow becomes visible at longer wavelengths after the jet has sufficiently decelerated and spread laterally. These events are referred to as orphan afterglows \citep{1999ApJ...513..656D}. When a jet is released, orphan afterglows can occur either because the GRB was outside the gamma-ray detector’s field of view or because the jet was initially misaligned with the observer’s line of sight, i.e., $\theta_{\text{view}} > \theta_j$ \citep{2003ApJ...591.1097R,2022Galax..10...93S}. While numerous candidates have been identified in the optical band \citep{2015ApJ...803L..24C,2020ApJ...905...98H}, only a single convincing orphan afterglow candidate has been discovered at radio wavelengths to date \citep{2018ApJ...866L..22L,2022ApJ...924...16M}.


\red{2. ASKAP is a wide-field radio interferometer consisting of 36 prime-focus antennas located at Inyarrimanha Ilgari Bundara / the CSIRO Murchison Radio-astronomy Observatory in Western Australia . It operates at frequencies between 700 and 1800\,MHz.   The discovery was based on four RACS epochs: two from RACS-low at 888 MHz (observed in 2019 and 2022), one from RACS-mid at 1367 MHz (observed in 2021; \citealt{2023PASA...40...34D}), and one from RACS-high at 1655 MHz \citep[2022;][]{2025PASA...42...38D}. We also include additional data from ten ASKAP epochs targeting the field of GW190814 \citep{2022MNRAS.510.3794D}, with significantly deeper sensitivity (RMS $\sim$35 $\mu$Jy) enabled by 10-hour integrations. We also used archival data from the VLASS survey (accessed via CIRADA\footnote{\url{https://cirada.ca/}}).}

Fluxes were computed with \texttt{PIMMS}\footnote{\url{https://url.au.m.mimecastprotect.com/s/pONmCOMKzVTvYJJpycEfMsG0qKk?domain=heasarc.gsfc.nasa.gov}} assuming a power-law spectrum with photon index $\Gamma=1.7$ and a Galactic line-of-sight absorption of $N_{\mathrm{H}}=2\times10^{20},\mathrm{cm^{-2}}$\footnote{calculated using the NASA HESARC NH calculator \url{https://heasarc.gsfc.nasa.gov/cgi-bin/Tools/w3nh/w3nh.pl}}, appropriate given the transient’s location outside the main body of the potential host galaxy. 

\blue{The source lacks both an infrared counterpart down to a depth of 23 mag (see Section \ref{ss:IR}) and an optical counterpart down to 28 mag (or 27 mag when host-galaxy extinction is accounted for; see Section \ref{sec:host_galaxy}), making a background AGN origin unlikely.}\blue{Despite its persistent radio emission, the source remains undetected in X-ray follow-up observations (see Section \ref{ss_xray}), with flux limits reaching the few nJy level. In addition, L-band observations with MeerKAT and data from the Parkes UWL telescope reveal no evidence of pulsed emission from pulsars in our own galaxy, disfavouring scenarios involving pulsars or gamma-ray binaries.}

\blue{We constrain circular polarisation to a $5\sigma$ upper limit on the fractional polarization (V/I) of 5.6\% using the 5.5\,GHz ATCA observation on 2023 June 8 ($S_V$=0.08\,mJy; $S_I$=1.39\,mJy).  We find no evidence of emission in Stokes $Q$, $U$, or $V$ in either observation, hence, not something stellar perhaps. }

\subsection{Radio Variability}
% \subsection{Interstellar Scintillation}


We measure a modulation index of $0.1 \pm 0.1$ and $0.3 \pm 0.3$ from the ATCA and ASKAP observations respectively, demonstrating all short-timescale variability to be consistent with noise. No variability is detected on minute timescales in either the ASKAP 0.9 GHz or ATCA 2.1 GHz (15-minute observations), despite expected diffractive timescales of 6.8 and 18.9 minutes, respectively, ruling out diffractive interstellar scintillation as the origin of the observed variability. But is detected at 0.9 GHz, meaning the source size should be less than $5\times 10^5$ uas. Since this is such a huge upper limit we carry out something mor esophisticated here to calculate what variability actually exists other than the observable.

Assuming ASKAP~J0055$-$2558 is a compact synchrotron source, its observed radio flux density is expected to be modulated by refractive interstellar scintillation (RISS; \citealt{2019arXiv190708395H}). To determine the amount of variability expected due to RISS, we use the NE2001 electron-density model \citep{2002astro.ph..7156C} at the Galactic coordinates of the source. The transition frequency between the strong and weak scattering regimes at the position of our transient is $\nu_0 = 7.46$\,GHz. Adopting the \citet{1998MNRAS.294..307W} formalism appropriate for extragalactic sources, we compute the angular size of the scattering disk, $\theta_r$, which sets the angular scale below which a source remains in the strong-scintillation regime at a given observing frequency (Table \ref{tab:iss_params}).

We estimate the source size via a preliminary equipartition analysis (Section~\ref{ss_eqipartition_analysis}) that does not include RISS errors. For all assumed geometries, the mean source size, $\theta_s$ is smaller than $\theta_r$ for $\nu \lesssim 2.3$GHz, whereas at 5.5GHz the mean source size exceeds $\theta_r$ for every geometry. At 3\,GHz, the $5^\circ$ conical geometry is an outlier relative to the less-collimated cases and lies above the scattering-disk size. Accordingly, we report modulation indices for two representative angular sizes: 190$\mu$as (less-collimated geometries) and 720~$\mu$as (the $5^\circ$ conical geometry). The modulation index, $m$, which quantifies the fractional flux variability due to RISS, is given by:

\begin{equation}
m = 
\begin{cases}
\left( \dfrac{\nu}{\nu_0} \right)^{17/30}, & \text{if } \theta_s \leq \theta_r,\theta_r = \theta_{F0} \left( \dfrac{\nu_0}{\nu} \right)^{11/5} \\
\left( \dfrac{\nu}{\nu_0} \right)^{17/30} \left( \dfrac{\theta_{r}}{\theta_s} \right)^{7/6}, & \text{if } \theta_s > \theta_r
\end{cases}
\end{equation}

\begin{deluxetable}{ccccc}
\tablecaption{Estimated RISS Parameters for ASKAP~J0055$-$2558 \label{tab:iss_params}}
\tablehead{
\colhead{$\nu$} & 
\colhead{$m_p$} & 
\colhead{$\theta_{F0}$} & 
\colhead{$\theta_r$} & 
\colhead{$m$} \\
\colhead{(GHz)} & 
\colhead{} & 
\colhead{($\mu$as)} & 
\colhead{($\mu$as)} & 
\colhead{}
}
\startdata
0.4 & 0.19 & 2076 & 1689745 & 0.19 \\
0.7 & 0.26 & 790  & 144024  & 0.26 \\
0.9 & 0.30 & 455  & 47720   & 0.30 \\
1.3 & 0.37 & 202  & 9434    & 0.37 \\
1.7 & 0.43 & 112  & 2899    & 0.43 \\
2.1 & 0.49 & 70   & 1138    & 0.49 \\
2.3 & 0.51 & 58   & 772     & 0.51 \\
3.0 & 0.60 & 32   & 237     & 0.60/0.16 \\
5.5 & 0.84 & 8    & 16      & 0.05/0.01 \\
9.0 & 0.76 & 3    & 2     & 0.01/0.001 \\\hline
% \end{tabular}
% \end{minipage}
% }
% \end{center}
\enddata
\tablecomments{Parameters include the point-source modulation index ($m_p$), Fresnel zone angular size ($\theta_{F0}$), scattering disk size ($\theta_r$), and final modulation index ($m$) accounting for source size. For $\nu \geq 3~\mathrm{GHz}$, two source sizes (190 and 772\,$\mu$as) are reported; for lower frequencies, $m$ is unchanged. Values are based on the NE2001 model and used to compute additional flux uncertainties from scintillation.}
\end{deluxetable}



where, $\theta_{F0}$ is the angular size of the first Fesnel zone. Before performing the spectral fitting, we add an extra uncertainty term to each flux density measurement to account for RISS, calculated as the modulation index (in percent) multiplied by the flux density. This is added in quadrature with the statistical measurement uncertainty to account for RISS-induced variability across frequencies and between epochs. This additional uncertainty varied from 19\% at 0.4 GHz to 51\% at 2.3 GHz and 1\% at 9 GHz in the weak regime. Because the uncertainty for the $5^\circ$ conical geometry is much smaller at 3 GHz and above, we adopted the larger uncertainty corresponding to the average source size of the less-collimated geometries for all spectral fitting. All additional uncertainties due to interstellar scintillation are reported in Table \ref{Table:Radio_obs}.




\blue{It is very unlikely that the $>20\times$ brightening in $\rm \source$ was an extreme scattering event (ESE): although large plasma lenses can in principle produce arbitrarily large magnification, $\mu \equiv S_{\rm obs}/S_{\rm int}$ \citep[e.g.][]{2016ApJ...817..176T}, the simultaneous high magnification typically spans only a narrow fractional bandwidth ($\Delta\nu/\nu \sim \mu^{-1}$) unless one invokes a contrived density profile. A broadband de-magnification from an over-focused lens could explain early non-detections and a modest trailing-horn enhancement \citep{1987Natur.326..675F,2016Sci...351..354B}, but the years-long decline at 9 and 5.5\,GHz with little variation below 2\,GHz argues against an ESE interpretation.}

\source\ exhibits a peaked radio spectrum in our broadband radio data. Such peaked spectra can arise from two generic mechanisms: (i) synchrotron self-absorption (SSA), in which the low-frequency turnover is intrinsic to a compact, recently activated (age $\lesssim 10^{5}$ yr) jet, lobe or blastwave \citep{chevalier_synchrotron_1998,1997AJ....113..148O,1998A&A...337...69O}; and (ii) free-free absorption (FFA), in which emission from the jet or lobe is attenuated by dense ionized plasma along the line of sight either homogeneous or inhomogenous \citep[for instance in Compact Steep Spectrum (CSS) and Gigahertz Peaked Spectrum (GPS) sources;][]{1984AJ.....89....5V}. In epochs with good low-frequency coverage we therefore fit the optically thick index as a free parameter, following \citet{2022MNRAS.512.5358R} to distinguish between these models. Among homogeneous FFA, inhomogeneous FFA, and SSA models, only SSA and inhomogeneous FFA reproduce the observed rising, optically thick spectrum of \source\ below the turnover, whereas homogeneous FFA predicts an exponential low-frequency cutoff inconsistent with the data.
Out of these two, we favour SSA due to several factors: the lack of IR/optical counterparts (unusual for GPS/CSS sources), a steep post-peak temporal decline faster than typical GPS/CSS evolution \citep{2016AN....337....9O,2022MNRAS.512.5358R}, and the low probability of chance alignment with a nearby star-forming galaxy (see section \ref{sec:host_galaxy}). However, an alternative, although unlikely, explanation is that \source\ is a heavily obscured background GPS/CSS object.

are weakly constrained, likely due to limited early-time coverage between the first low frequency detections and multifrequency follow-up.

It is very unlikely that the significant, over a factor of 20, brightening observed in \source is due to an extreme scattering event (ESE). While there is essentially no limit on the magnification $\mu$ due to lensing by a large-scale plasma lens \citep[\textit{e.g.},][]{2016ApJ...817..176T}, the fractional bandwidth of simultaneous high magnification is expected to be low, of order $\Delta\nu/\nu\propto1/\mu$, unless a highly contrived plasma density profile is invoked.

Specifically, one can write for the magnification of an image as a function of frequency:
\begin{equation}
    \mu(\nu)=\left|1-2\frac{\nu_0^2}{\nu^2}\kappa+\frac{\nu_0^4}{\nu^4}(\kappa^2-\gamma^2)\right|^{-1}
\end{equation}
with $\kappa$ and $\gamma$ combinations of the second derivatives of the plasma column, and maintaining high magnification over a broad range of $\nu$ requires the last two terms on the right-hand side to keep a value very near 1 over that range. While $\kappa, \gamma$ themselves depend on frequency via the chromaticity in the position of the image, the latter is determined from an equation involving first derivatives of the column. Thus, although it is in principle possible to fit an arbitrary (sufficiently smooth) dynamic spectrum with a 2D plasma lens, it would require a highly unnatural plasma arrangement.

It is significantly easier to achieve broadband \emph{de}-magnification using a highly overfocused lens -- \textit{i.e.}, where $|\kappa|$ and/or $\gamma$ are well in excess of unity at the centre of the required band. This would imply interpreting non-detections in early epochs as due to de-magnification and subsequent brightening as return to its intrinsic brightness, possibly undergoing a modest enhancement in the trailing 'horn' of the classic ESE light curve \citep{1987Natur.326..675F}. The light curves shown in Figure~\ref{fig:lightcurve} are consistent with the higher-to-lower frequencies direction of the caustic sweep expected in the trailing half of the ESE \citep{2016Sci...351..354B} and lack of constraints on the\source ASKAP~J0055-2558 brightness prior to 2019 or its intrinsic spectrum does not allow to rule out this scenario completely. However, the continuing decline of 9 GHz and 5.5 GHz light curves years after their presumed peak with little variation of flux below 2 GHz makes this interpretation increasingly unlikely.

It is also very unlikely that the $>20\times$ brightening in \source\ was an extreme scattering event (ESE): while large plasma lenses can in principle yield high magnification \citep[e.g.][]{2016ApJ...817..176T}, the simultaneous high magnification, $\mu$, typically spans only a narrow fractional bandwidth ($\Delta\nu/\nu\sim\mu^{-1}$) unless a contrived lens profile is invoked. A broadband de-magnification followed by a brief enhancement could mimic early non-detections and a trailing horn \citep{1987Natur.326..675F,2016Sci...351..354B}, but the years-long, broadband decline (strong at 5.5 and 9\,GHz with little variation below 2\,GHz) rules out an ESE origin.

Imaging was done with w-projection algorithm convolution to correct for the widefield
non-coplanar baseline effect \citep{2008ISTSP...2..647C} and a Briggs robust parameter of zero that provides a higher angular resolution than natural weighting while slightly increasing the image noise. At the low frequencies the uGMRT operates at, the ionosphere introduces propagation delay differences between the elements in the array, introducing phase errors \citep{2019MNRAS.483.1184M}. Self-calibration is a common method to account for this, which involves calibrating the data using the multiple compact and bright sources in the original model image and then re-imaging the corrected data in an iterative process to create better models \citep{1984ARA&A..22...97P}. We applied four phase-only self-calibration cycles (solution intervals: 4, 2, 1 and 0.5 min) and four amplitude and phase self-calibration cycles (solution intervals: 8, 4, 2 and 1 min) to the target visibilities. 


 We first constructed a point spread function (PSF) model by identifying all stars in the image detected at a significance of $>10\sigma$  and taking a weighted mean stack of cutouts of the stars.


 

We conducted an equipartition analysis to infer physical properties of the synchrotron-emitting region from spectral observations, following the methods of \citet{2013ApJ...772...78B} and the code published in \citet{2022MNRAS.511.5328G,2023MNRAS.518..847G}. Using the observed spectral $\nu_p$, $F_p$, and $\alpha_2$, and distance luminosity of the potential host galaxy, $d_L=543 \rm \,Mpc$, we derived the radius ($R$), energy ($E$), velocity ($\beta$), magnetic field ($B$), and electron density ($n_e$). We consider both spherical and conical geometries: the spherical case assumes $f_A = 1$ and $f_V = 4/3$. \blue{For the conical outflow geometry, we consider two components: (i) two narrowly collimated relativistic jets with Lorentz factor $\Gamma=10$ and half-opening angle $\theta_j\leq10^\circ$, and (ii) a wide-angle, non-relativistic outflow. In all cases, the area filling factor $f_A$ is computed from the half-opening angle ($\theta_j=\Theta/2$). For the narrow relativistic jets we adopt $f_A=f_V=\Gamma,\theta_{j,\mathrm{rad}}^2$ \citep{2013ApJ...772...78B}, while for the wide-angle outflow we use the geometric expression $f_A=1-\cos\theta_j$ and fix the volume filling factor at $f_V=1.0$, following the standard unit-volume convention in non-relativistic equipartition models \citep{2016ApJ...819L..25A,2024MNRAS.528.7123G}. For opening angles($\Theta$) of $5^\circ$, $15^\circ$, and $30^\circ$, this yields $f_A=f_V=0.019$, $f_A=f_V=0.17$, and $f_A=0.034$ with $f_V=1.0$, respectively.} 


% \begin{equation}
% \begin{aligned}
% F(\nu,t) &= A(t)\,\left[\left(\frac{\nu}{\nu_b(t)}\right)^{-s\alpha_1}
%            + \left(\frac{\nu}{\nu_b(t)}\right)^{-s\alpha_2}\right]^{-\frac{1}{s}},\\[4pt] 
% \nu_b(t) &= \nu_{b,0}\left(\frac{t}{t_0}\right)^{m},
% A(t) = A_0\,\frac{F(t)}{F(t_0)},\\[4pt], F(t) &= \left[\left(\frac{t}{t_b}\right)^{-s_t b_1} + \left(\frac{t}{t_b}\right)^{-s_t b_2}\right]^{-\frac{1}{s_t}}\\[6pt]
% \end{aligned}
% \end{equation}

The amplitude $A(t)$ transitions between temporal slopes $b_1$ and $b_2$ around the break time $t_b$ with smoothness $s_t$, and is normalised so that $A(t_0)=A_0$ at the reference epoch $t_0$.


% \subsection{Event Rates Comparison}

% To further assess the nature of the transient, we compare the inferred volumetric event rate for this source with the rates of the two most plausible interpretations: jetted off-nuclear TDE involving an IMBH, and an orphan afterglow of a l-GRB, observed either on or off-axis. We estimate the volumetric event rate using the survey sensitivity, $F_{\nu,\mathrm{lim}}$, of 0.15\,mJy (most constraining from the AS111 observation), an effective search area of 22\,deg$^2$ (corresponding to the 90\% localization region of GW190814; solid angle, $\Omega = 5.3\times10^{-4}$), a host distance,  of 543\,Mpc ($z \sim 0.116$; $\rm L_{\nu,\mathrm{peak}}\approx10^{29}\:erg\:s^{-1}\:Hz$), and a detectable transient evolution timescale of 3 years, 

% \begin{equation}
%     \mathscr{R} = \frac{1\:\mathrm{event}}{V \cdot T}, \quad
%     V = \frac{\Omega\, d_{L,\mathrm{max}}^3}{3}, \quad
%     d_{L,\mathrm{max}} = \left[\frac{L_{\nu,\mathrm{peak}}}{4\pi F_{\nu,\mathrm{lim}}}\right]^{1/2}
% \end{equation}

% This yields a volumetric rate for the transient of $\mathscr{R} \approx 11.35\,\mathrm{Gpc^{-3}\,yr^{-1}}$. This estimated rate for \source\ is consistent with predictions for off-axis long GRBs \citep[$\mathscr{R} \sim 3\,\mathrm{Gpc^{-3}\,yr^{-1}}$;][]{2014PASA...31...22G} and for off-nuclear jetted TDEs \citep[$\mathscr{R} \sim 1$–$10\,\mathrm{Gpc^{-3}\,yr^{-1}}$;][]{2025ApJ...980L..22C}. However, it is somewhat inconsistent with the higher rate expected for on-axis GRBs (total l-GRB rate: $\mathscr{R} = 79^{+57}_{-33}\,\mathrm{Gpc^{-3}\,yr^{-1}}$; $<3\%$ off-axis at $z < 2$), assuming one was missed solely due to lack of detector coverage \citep{2022ApJ...932...10G}. This comparison provides an additional constraint on the progenitor scenario of the observed transient, favouring models with intrinsically lower observable rates, such as off-axis GRBs or off-nuclear jetted TDEs.
